Driftfusion: An open source code for simulating ordered semiconductor devices with mixed ionic-electronic conducting materials in one-dimension

The recent emergence of lead-halide perovskites as active layer materials for thin film semiconductor devices including solar cells, light emitting diodes, and memristors has motivated the development of several new drift-diffusion models that include the effects of both mobile electronic and ionic charge carriers. The aim of this work is to provide a comprehensive guide to Driftfusion, a versatile simulation tool built for simulating one-dimensional ordered semiconductor devices with mixed ionic-electronic conducting layers. Driftfusion enables users to model devices with multiple, distinct, material layers and up to four charge carrier species: electrons and holes by default plus up to two ionic species. The time-dependent carrier continuity equations are fully-coupled to Poisson's equation enabling transient optoelectronic device measurement protocols to be simulated. In addition to material and device-wide properties, users have direct access to adapt the physical models for carrier transport, generation and recombination. Furthermore, a graded-interface approach circumvents the requirement for boundary conditions at material interfaces and enables interface-specific properties, such as high rates of interfacial recombination, to be introduced.

==> 2019 Driftfusion methods arXiv submission 2/Lst1_Equation_editor.tex <==
function solstruct = df(varargin)
% Core DRIFTFUSION function- organises properties and inputs for pdepe
% A routine to test solving the diffusion and drift equations using the
% matlab pepde solver.
%
%% LICENSE
% Copyright (C) 2020  Philip Calado, Ilario Gelmetti, and Piers R. F. Barnes
% Imperial College London
% This program is free software: you can redistribute it and/or modify
% it under the terms of the GNU Affero General Public License as published
% by the Free Software Foundation, either version 3 of the License, or
% (at your option) any later version.
%
% Solution outputs
% V = u(1) = electrostatic potential
% n = u(2) = electron density
% p = u(3) = holes density
% c = u(4) = cation density (optional)
% a = u(5) = anion density (optional)
%
%% Start code
%% Deal with input arguments
if length(varargin) == 0
    % If no input parameter set then call pc directly
    par = pc;
    dficAnalytical = true;
elseif length(varargin) == 1
    % If one input argument then assume it is the Initial Conditions (IC) solution
    icsol = varargin{1, 1}.u;
    icx = varargin{1, 1}.x;
    par = varargin{1, 1}.par;
    dficAnalytical = false;
elseif length(varargin) == 2
    if max(max(max(varargin{1, 1}.u))) == 0
        par = varargin{2};
        dficAnalytical = true;
    elseif isa(varargin{2}, 'char') == 1            % Checks to see if argument is a character
        input_solstruct = varargin{1, 1};
        par = input_solstruct.par;
        icsol = input_solstruct.u;
        icx = input_solstruct.x;
        dficAnalytical = false;
    else
        input_solstruct = varargin{1, 1};
        icsol = input_solstruct.u;
        icx = input_solstruct.x;
        par = varargin{2};
        dficAnalytical = false;
    end
end

%% Unpack properties
%% Spatial mesh
xmesh = par.xx;
x_sub = par.x_sub;
x = xmesh;

%% Time mesh
t = meshgen_t(par);

%% Dependent properties: Prevents recalculation of dependent properties by pdepe defined in Methods
% Can also use AbortSet in class def
Vbi = par.Vbi;
nleft = par.nleft;
nright = par.nright;
pleft = par.pleft;
pright = par.pright;
dev = par.dev;

%% Constants
kB = par.kB;
q = par.q;
e = par.e;
epp0 = par.epp0;

%% Device parameters
device = par.dev_sub;
T = par.T;
mue = device.mue;           % Electron mobility
muh = device.muh;           % Hole mobility
Dn = mue*kB*T;              % Electron diffusion coefficient
Dp = muh*kB*T;              % Hole diffusion coefficient
mucat = device.mucat;       % Cation mobility
muani = device.muani;       % Anion mobility
Nc = device.Nc;             % Conduction band effective density of states
Nv = device.Nv;             % Valence band effective density of states
cmax = device.cmax;     % Cation density upper limit
amax = device.amax;     % Anion density upper limit
gradNc = device.gradNc;     % Conduction band effective density of states gradient
gradNv = device.gradNv;     % Valence band effective density of states gradient
gradEA = device.gradEA;     % Electron Affinity gradient
gradIP = device.gradIP;     % Ionisation Potential gradient
epp = device.epp;           % Dielectric constant
eppmax = max(par.epp);      % Maximum dielectric constant (for normalisation)
B = device.B;               % Radiative recombination rate coefficient
ni = device.ni;             % Intrinsic carrier density
taun = device.taun;         % Electron SRH time constant
taup = device.taup;         % Electron SRH time constant
taun_vsr = device.taun_vsr; % Electron SRH time constant- volumetric interfacial surface recombination scheme
taup_vsr = device.taup_vsr; % Electron SRH time constant- volumetric interfacial surface recombination scheme
nt = device.nt;             % SRH electron trap constant
pt = device.pt;             % SRH hole trap constant
NA = device.NA;             % Acceptor doping density
ND = device.ND;             % Donor doping density
Ncat = device.Ncat;         % Uniform cation density
Nani = device.Nani;         % Uniform anion density
xprime_n = device.xprime_n;         % Translated x co-ordinates for interfaces
xprime_p = device.xprime_p;         % Translated x co-ordinates for interfaces
sign_xn = device.sign_xn;           % 1 if xn increasing, -1 if decreasing wrt x
sign_xp = device.sign_xp;           % 1 if xp increasing, -1 if decreasing wrt x
alpha0_xn = device.alpha0_xn;       % alpha0_xn is alpha for F = 0 reference to xprime_n
beta0_xp = device.beta0_xp;         % beta0_xp is beta for F = 0 referenced to xprime_p
N_max_variables = par.N_max_variables;  % Maximum number of variables allowable in this version of Driftfusion
N_ionic_species = par.N_ionic_species;  % Number of ionic species in this solution
N_variables = par.N_ionic_species + 3;  % Number of variables in this solution (+3 for V, n, and p)

z_c = par.z_c;
z_a = par.z_a;
nleft = par.nleft;
nright = par.nright;
pleft = par.pleft;
pright = par.pright;
sn_l = par.sn_l;
sp_l = par.sp_l;
sn_r = par.sn_r;
sp_r = par.sp_r;
Rs = par.Rs;
Rs_initial = par.Rs_initial;

%% Switches and accelerator coefficients
mobset = par.mobset;        % Electronic carrier transport switch
mobseti = par.mobseti;      % Ionic carrier transport switch
K_cation = par.K_cation;    % Cation transport rate multiplier
K_anion = par.K_anion;      % Anion transport rate multiplier
radset = par.radset;        % Radiative recombination switch
SRHset = par.SRHset;        % SRH recombination switch
vsr_zone = device.vsr_zone;
srh_zone = device.vsr_zone;
Field_switch = device.Field_switch;

%% Generation
g1_fun = fun_gen(par.g1_fun_type);
g2_fun = fun_gen(par.g2_fun_type);
gxt1 = 0;
gxt2 = 0;
g = 0;
gx1 = par.gx1;
gx2 = par.gx2;
int1 = par.int1;
int2 = par.int2;
g1_fun_type = par.g1_fun_type;
g2_fun_type = par.g2_fun_type;
g1_fun_arg = par.g1_fun_arg;
g2_fun_arg = par.g2_fun_arg;

%% Voltage function
Vapp_fun = fun_gen(par.V_fun_type);
Vapp = 0;
Vres = 0;
J = 0;

%% Solver variables
V = 0; n = 0; p = 0; a = 0; c = 0;
dVdx = 0; dndx = 0; dpdx = 0; dadx = 0; dcdx = 0;
C_V = 0; C_n = 0; C_p = 0; C_c = 0; C_a = 0;
F_V = 0; F_n = 0; F_p = 0; F_c = 0; F_a = 0;
S_V = 0; S_n = 0; S_p = 0; S_c = 0; S_a = 0;
r_rad = 0; r_srh = 0; r_vsr = 0; r_np = 0;
alpha = 0; beta = 0;

%% Solver options
% MaxStep = limit maximum time step size during integration
options = odeset('MaxStep', par.MaxStepFactor*0.1*abs(par.tmax - par.t0), 'RelTol', par.RelTol, 'AbsTol', par.AbsTol, 'NonNegative', [1,1,1,0]);

%% Call solver
% inputs with '@' are function handles to the subfunctions
% below for the: equation, initial conditions, boundary conditions
u = pdepe(par.m,@dfpde,@dfic,@dfbc,x,t,options);

%% Ouputs
% Store final voltage reading
par.Vapp = Vapp;

% Solutions and meshes to structure
solstruct.u = u;
solstruct.x = x;
solstruct.t = t;

% Store parameters object
solstruct.par = par;

%% Volumetric surface recombination error check
if par.vsr_mode == 1 && par.vsr_check == 1
    compare_rec_flux(solstruct, par.RelTol_vsr, par.AbsTol_vsr, 0);
end

%% Subfunctions
% Set up partial differential equation (pdepe) (see MATLAB pdepe help for details of C,F,S)
% C = Time-dependence prefactor
% F = Flux terms
% S = Source terms
    function [C,F,S] = dfpde(x,t,u,dudx)
        % Get position point
        i = find(x_sub <= x);
        i = i(end);

        switch g1_fun_type
            case 'constant'
                gxt1 = int1*gx1(i);
            otherwise
                gxt1 = g1_fun(g1_fun_arg, t)*gx1(i);
        end

        switch g2_fun_type
            case 'constant'
                gxt2 = int2*gx2(i);
            otherwise
                gxt2 = g2_fun(g2_fun_arg, t)*gx2(i);
        end
        g = gxt1 + gxt2;

        %% Unpack Variables
        
        
                V = u(1);
                n = u(2);
                p = u(3);
                c = u(4);
                a = u(5);
                dVdx = dudx(1);
                dndx = dudx(2);
                dpdx = dudx(3);
                dcdx = dudx(4);
                dadx = dudx(5);












%% Equation editor
% Time-dependence prefactor term
C_V = 0; C_n = 1; C_p = 1; C_c = 1; C_a = 1;
C = [C_V; C_n; C_p; C_c; C_a];

% Flux terms
F_V = (epp(i)/eppmax)*dVdx;
F_n = mu_n(i)*n*(-dVdx + gradEA(i)) + (Dn(i)*(dndx - ((n/Nc(i))*gradNc(i))));
F_p = mu_p(i)*p*(dVdx - gradIP(i)) + (Dp(i)*(dpdx - ((p/Nv(i))*gradNv(i))));
F_c = mu_c(i)*(z_c*c*dVdx + kB*T*(dcdx + (c*(dcdx/(c_max(i) - c)))));
F_a = mu_a(i)*(z_a*a*dVdx + kB*T*(dadx + (a*(dadx/(a_max(i) - a)))));
F = [F_V; mobset*F_n; mobset*F_p; mobseti*K_c*F_c; mobseti*K_a*F_a];

% Electron and hole recombination
% Radiative
r_rad = radset*B(i)*(n*p - ni(i)^2);
% Bulk SRH
r_srh = SRHset*srh_zone(i)*((n*p - ni(i)^2)/(taun(i)*(p + pt(i)) + taup(i)*(n + nt(i))));
% Volumetric surface recombination
alpha = sign_xn(i)*q*dVdx/(kB*T) + alpha0_xn(i);
beta = sign_xp(i)*q*-dVdx/(kB*T) + beta0_xp(i);
r_vsr = SRHset*vsr_zone(i)*((n*exp(-alpha*xprime_n(i))*p*exp(-beta*xprime_p(i)) - ni(i)^2)...
    /(taun_vsr(i)*(p*exp(-beta*xprime_p(i)) + pt(i)) + taup_vsr(i)*(n*exp(-alpha*xprime_n(i)) + nt(i))));
% Total electron and hole recombination
r_np = r_rad + r_srh + r_vsr;

% Source terms
S_V = (q/(eppmax*epp0))*(-n + p - NA(i) + ND(i) + z_a*a + z_c*c - z_a*Nani(i) - z_c*Ncat(i));
S_n = g - r_np;
S_p = g - r_np;
S_c = 0;
S_a = 0;
S = [S_V; S_n; S_p; S_c; S_a];

        % Remove unused variables - faster and tidier than using conditional
        % statements
        C = C(1:N_variables);
        F = F(1:N_variables);
        S = S(1:N_variables);
    end

%% Initial conditions.
    function u0 = dfic(x)
        i = find(xmesh <= x);
        i = i(end);

        if length(par.dcell) == 1
            % Single layer
            u0_ana = [(x/xmesh(end))*Vbi;
                nleft*exp((x*(log(nright)-log(nleft)))/par.dcum0(end));
                pleft*exp((x*(log(pright)-log(pleft)))/par.dcum0(end));
                dev.Ncat(i);
                dev.Nani(i);];
        else
            % Multi-layered
            u0_ana = [(x/xmesh(end))*Vbi;
                dev.n0(i);
                dev.p0(i);
                dev.Ncat(i);
                dev.Nani(i);];
        end
        u0_ana = u0_ana(1:N_variables);

        % Organise ICs based on number of variables and SOL_IC
        if dficAnalytical
            u0 = u0_ana;
        else
            % Initial conditions taken from input solution
            u0_in = interp1(icx,squeeze(icsol(end,:,:)),x)';
            % If the number of variables has increased then add analytical
            % ICs for missing variables
            if N_variables > length(u0_in)
                % Add initial conditions for new variables from U_ANA
                u0(1:length(u0_in), 1) = u0_in;
                u0(length(u0_in)+1:N_variables, 1) = u0_ana(length(u0_in)+1:N_variables);
            else
                u0 = u0_in;
            end
        end
    end

%% Boundary conditions
% Refer to PDEPE help for the precise meaning of P and Q
% l and r refer to left and right boundaries.
    function [Pl,Ql,Pr,Qr] = dfbc(xl,ul,xr,ur,t)

        switch N_ionic_species
            case 0
                V_l = ul(1);
                V_r = ur(1);
                n_l = ul(2);
                n_r = ur(2);
                p_l = ul(3);
                p_r = ur(3);
                c_l = 0;
                c_r = 0;
                a_l = 0;
                a_r = 0;
            case 1
                V_l = ul(1);
                V_r = ur(1);
                n_l = ul(2);
                n_r = ur(2);
                p_l = ul(3);
                p_r = ur(3);
                c_l = ul(4);
                c_r = ur(4);
                a_l = 0;
                a_r = 0;
            case 2
                V_l = ul(1);
                V_r = ur(1);
                n_l = ul(2);
                n_r = ur(2);
                p_l = ul(3);
                p_r = ur(3);
                c_l = ul(4);
                c_r = ur(4);
                a_l = ul(5);
                a_r = ur(5);
        end

        switch par.V_fun_type
            case 'constant'
                Vapp = par.V_fun_arg(1);
            otherwise
                Vapp = Vapp_fun(par.V_fun_arg, t);
        end

                % Flux boundary conditions for both carrier types.
                % Calculate series resistance voltage Vres
                if Rs == 0
                    Vres = 0;
                else
                    J = e*sp_r*(ur(3) - pright) - e*sn_r*(ur(2) - nright);
                    if Rs_initial
                        Vres = -J*Rs*t/par.tmax;    % Initial linear sweep
                    else
                        Vres = -J*Rs;
                    end
                end

Pl = [-V_l;
  mobset*(-sn_l*(n_l - n0_l));
  mobset*(-sp_l*(p_l - p0_l));
  0;
  0;];

Ql = [0; 1; 1; 1; 1;];

Pr = [-V_r+Vbi-Vapp-Vres;
  mobset*(sn_r*(n_r - n0_r));
  mobset*(sp_r*(p_r - p0_r));
  0;
  0;];

Qr = [0; 1; 1; 1; 1;];


        % Remove unused entries
        Pl = Pl(1:N_variables);
        Pr = Pr(1:N_variables);
        Ql = Ql(1:N_variables);
        Qr = Qr(1:N_variables);
    end
end


==> 2019 Driftfusion methods arXiv submission 2/Lst2_dfbc.tex <==
function solstruct = df(varargin)
% Core DRIFTFUSION function- organises properties and inputs for pdepe
% A routine to test solving the diffusion and drift equations using the
% matlab pepde solver.
%
%% LICENSE
% Copyright (C) 2020  Philip Calado, Ilario Gelmetti, and Piers R. F. Barnes
% Imperial College London
% This program is free software: you can redistribute it and/or modify
% it under the terms of the GNU Affero General Public License as published
% by the Free Software Foundation, either version 3 of the License, or
% (at your option) any later version.
%
% Solution outputs
% V = u(1) = electrostatic potential
% n = u(2) = electron density
% p = u(3) = holes density
% c = u(4) = cation density (optional)
% a = u(5) = anion density (optional)
%
%% Start code
%% Deal with input arguments
if length(varargin) == 0
    % If no input parameter set then call pc directly
    par = pc;
    dficAnalytical = true;
elseif length(varargin) == 1
    % If one input argument then assume it is the Initial Conditions (IC) solution
    icsol = varargin{1, 1}.u;
    icx = varargin{1, 1}.x;
    par = varargin{1, 1}.par;
    dficAnalytical = false;
elseif length(varargin) == 2
    if max(max(max(varargin{1, 1}.u))) == 0
        par = varargin{2};
        dficAnalytical = true;
    elseif isa(varargin{2}, 'char') == 1            % Checks to see if argument is a character
        input_solstruct = varargin{1, 1};
        par = input_solstruct.par;
        icsol = input_solstruct.u;
        icx = input_solstruct.x;
        dficAnalytical = false;
    else
        input_solstruct = varargin{1, 1};
        icsol = input_solstruct.u;
        icx = input_solstruct.x;
        par = varargin{2};
        dficAnalytical = false;
    end
end

%% Unpack properties
%% Spatial mesh
xmesh = par.xx;
x_sub = par.x_sub;
x = xmesh;

%% Time mesh
t = meshgen_t(par);

%% Dependent properties: Prevents recalculation of dependent properties by pdepe defined in Methods
% Can also use AbortSet in class def
Vbi = par.Vbi;
nleft = par.nleft;
nright = par.nright;
pleft = par.pleft;
pright = par.pright;
dev = par.dev;

%% Constants
kB = par.kB;
q = par.q;
e = par.e;
epp0 = par.epp0;

%% Device parameters
device = par.dev_sub;
T = par.T;
mue = device.mue;           % Electron mobility
muh = device.muh;           % Hole mobility
Dn = mue*kB*T;              % Electron diffusion coefficient
Dp = muh*kB*T;              % Hole diffusion coefficient
mucat = device.mucat;       % Cation mobility
muani = device.muani;       % Anion mobility
Nc = device.Nc;             % Conduction band effective density of states
Nv = device.Nv;             % Valence band effective density of states
cmax = device.cmax;     % Cation density upper limit
amax = device.amax;     % Anion density upper limit
gradNc = device.gradNc;     % Conduction band effective density of states gradient
gradNv = device.gradNv;     % Valence band effective density of states gradient
gradEA = device.gradEA;     % Electron Affinity gradient
gradIP = device.gradIP;     % Ionisation Potential gradient
epp = device.epp;           % Dielectric constant
eppmax = max(par.epp);      % Maximum dielectric constant (for normalisation)
B = device.B;               % Radiative recombination rate coefficient
ni = device.ni;             % Intrinsic carrier density
taun = device.taun;         % Electron SRH time constant
taup = device.taup;         % Electron SRH time constant
taun_vsr = device.taun_vsr; % Electron SRH time constant- volumetric interfacial surface recombination scheme
taup_vsr = device.taup_vsr; % Electron SRH time constant- volumetric interfacial surface recombination scheme
nt = device.nt;             % SRH electron trap constant
pt = device.pt;             % SRH hole trap constant
NA = device.NA;             % Acceptor doping density
ND = device.ND;             % Donor doping density
Ncat = device.Ncat;         % Uniform cation density
Nani = device.Nani;         % Uniform anion density
xprime_n = device.xprime_n;         % Translated x co-ordinates for interfaces
xprime_p = device.xprime_p;         % Translated x co-ordinates for interfaces
sign_xn = device.sign_xn;           % 1 if xn increasing, -1 if decreasing wrt x
sign_xp = device.sign_xp;           % 1 if xp increasing, -1 if decreasing wrt x
alpha0_xn = device.alpha0_xn;       % alpha0_xn is alpha for F = 0 reference to xprime_n
beta0_xp = device.beta0_xp;         % beta0_xp is beta for F = 0 referenced to xprime_p
N_max_variables = par.N_max_variables;  % Maximum number of variables allowable in this version of Driftfusion
N_ionic_species = par.N_ionic_species;  % Number of ionic species in this solution
N_variables = par.N_ionic_species + 3;  % Number of variables in this solution (+3 for V, n, and p)

z_c = par.z_c;
z_a = par.z_a;
nleft = par.nleft;
nright = par.nright;
pleft = par.pleft;
pright = par.pright;
sn_l = par.sn_l;
sp_l = par.sp_l;
sn_r = par.sn_r;
sp_r = par.sp_r;
Rs = par.Rs;
Rs_initial = par.Rs_initial;

%% Switches and accelerator coefficients
mobset = par.mobset;        % Electronic carrier transport switch
mobseti = par.mobseti;      % Ionic carrier transport switch
K_cation = par.K_cation;    % Cation transport rate multiplier
K_anion = par.K_anion;      % Anion transport rate multiplier
radset = par.radset;        % Radiative recombination switch
SRHset = par.SRHset;        % SRH recombination switch
vsr_zone = device.vsr_zone;
srh_zone = device.vsr_zone;
Field_switch = device.Field_switch;

%% Generation
g1_fun = fun_gen(par.g1_fun_type);
g2_fun = fun_gen(par.g2_fun_type);
gxt1 = 0;
gxt2 = 0;
g = 0;
gx1 = par.gx1;
gx2 = par.gx2;
int1 = par.int1;
int2 = par.int2;
g1_fun_type = par.g1_fun_type;
g2_fun_type = par.g2_fun_type;
g1_fun_arg = par.g1_fun_arg;
g2_fun_arg = par.g2_fun_arg;

%% Voltage function
Vapp_fun = fun_gen(par.V_fun_type);
Vapp = 0;
Vres = 0;
J = 0;

%% Solver variables
V = 0; n = 0; p = 0; a = 0; c = 0;
dVdx = 0; dndx = 0; dpdx = 0; dadx = 0; dcdx = 0;
C_V = 0; C_n = 0; C_p = 0; C_c = 0; C_a = 0;
F_V = 0; F_n = 0; F_p = 0; F_c = 0; F_a = 0;
S_V = 0; S_n = 0; S_p = 0; S_c = 0; S_a = 0;
r_rad = 0; r_srh = 0; r_vsr = 0; r_np = 0;
alpha = 0; beta = 0;

%% Solver options
% MaxStep = limit maximum time step size during integration
options = odeset('MaxStep', par.MaxStepFactor*0.1*abs(par.tmax - par.t0), 'RelTol', par.RelTol, 'AbsTol', par.AbsTol, 'NonNegative', [1,1,1,0]);

%% Call solver
% inputs with '@' are function handles to the subfunctions
% below for the: equation, initial conditions, boundary conditions
u = pdepe(par.m,@dfpde,@dfic,@dfbc,x,t,options);

%% Ouputs
% Store final voltage reading
par.Vapp = Vapp;

% Solutions and meshes to structure
solstruct.u = u;
solstruct.x = x;
solstruct.t = t;

% Store parameters object
solstruct.par = par;

%% Volumetric surface recombination error check
if par.vsr_mode == 1 && par.vsr_check == 1
    compare_rec_flux(solstruct, par.RelTol_vsr, par.AbsTol_vsr, 0);
end

%% Subfunctions
% Set up partial differential equation (pdepe) (see MATLAB pdepe help for details of C,F,S)
% C = Time-dependence prefactor
% F = Flux terms
% S = Source terms
    function [C,F,S] = dfpde(x,t,u,dudx)
        % Get position point
        i = find(x_sub <= x);
        i = i(end);

        switch g1_fun_type
            case 'constant'
                gxt1 = int1*gx1(i);
            otherwise
                gxt1 = g1_fun(g1_fun_arg, t)*gx1(i);
        end

        switch g2_fun_type
            case 'constant'
                gxt2 = int2*gx2(i);
            otherwise
                gxt2 = g2_fun(g2_fun_arg, t)*gx2(i);
        end
        g = gxt1 + gxt2;

        %% Unpack Variables
        switch N_ionic_species
            case 0
                V = u(1);
                n = u(2);
                p = u(3);
                c = 0;
                a = 0;
                dVdx = dudx(1);
                dndx = dudx(2);
                dpdx = dudx(3);
                dcdx = 0;
                dadx = 0;
            case 1
                V = u(1);
                n = u(2);
                p = u(3);
                c = u(4);
                a = Nani(i);
                dVdx = dudx(1);
                dndx = dudx(2);
                dpdx = dudx(3);
                dcdx = dudx(4);
                dadx = 0;
            case 2
                V = u(1);
                n = u(2);
                p = u(3);
                c = u(4);
                a = u(5);
                dVdx = dudx(1);
                dndx = dudx(2);
                dpdx = dudx(3);
                dcdx = dudx(4);
                dadx = dudx(5);
        end

        % Volumetric surface recombination gradients
        alpha = sign_xn(i)*q*dVdx/(kB*T) + alpha0_xn(i);
        beta = sign_xp(i)*q*-dVdx/(kB*T) + beta0_xp(i);

        %% Equation editor
        % Time-dependence prefactor term
        C_V = 0;
        C_n = 1;
        C_p = 1;
        C_c = 1;
        C_a = 1;
        C = [C_V; C_n; C_p; C_c; C_a];

        % Flux terms
        F_V = (epp(i)/eppmax)*dVdx;
        F_n = mue(i)*n*(-dVdx + gradEA(i)) + (Dn(i)*(dndx - ((n/Nc(i))*gradNc(i))));
        F_p = muh(i)*p*(dVdx - gradIP(i)) + (Dp(i)*(dpdx - ((p/Nv(i))*gradNv(i))));
        F_c = mucat(i)*(z_c*c*dVdx + kB*T*(dcdx + (c*(dcdx/(cmax(i)-c)))));
        F_a = muani(i)*(z_a*a*dVdx + kB*T*(dadx+(a*(dadx/(amax(i)-a)))));
        F = [F_V; mobset*F_n; mobset*F_p; K_cation*mobseti*F_c; K_anion*mobseti*F_a];

        % Electron and holes recombination
        % Radiative
        r_rad = radset*B(i)*((n*p)-(ni(i)^2));
        % Bulk SRH
        r_srh = SRHset*srh_zone(i)*(((n*p)-ni(i)^2)/(taun(i)*(p+pt(i)) + taup(i)*(n+nt(i))));
        % Volumetric surface recombination
        r_vsr = SRHset*vsr_zone(i)*((n*exp(-alpha*xprime_n(i))*p*exp(-beta*xprime_p(i)) - ni(i)^2)...
            /(taun_vsr(i)*(p*exp(-beta*xprime_p(i))+pt(i)) + taup_vsr(i)*(n*exp(-alpha*xprime_n(i))+nt(i))));
        % Total electron and hole recombination
        r_np = r_rad + r_srh + r_vsr;

        % Source terms
        S_V = Field_switch(i)*(q/(eppmax*epp0))*(-n + p - NA(i) + ND(i) + z_a*a + z_c*c);
        S_n = g - r_np;
        S_p = g - r_np;
        S_c = 0;
        S_a = 0;
        S = [S_V; S_n; S_p; S_c; S_a];

        % Remove unused variables - faster and tidier than using conditional
        % statements
        C = C(1:N_variables);
        F = F(1:N_variables);
        S = S(1:N_variables);
    end

%% Initial conditions.
    function u0 = dfic(x)
        i = find(xmesh <= x);
        i = i(end);

        if length(par.dcell) == 1
            % Single layer
            u0_ana = [(x/xmesh(end))*Vbi;
                nleft*exp((x*(log(nright)-log(nleft)))/par.dcum0(end));
                pleft*exp((x*(log(pright)-log(pleft)))/par.dcum0(end));
                dev.Ncat(i);
                dev.Nani(i);];
        else
            % Multi-layered
            u0_ana = [(x/xmesh(end))*Vbi;
                dev.n0(i);
                dev.p0(i);
                dev.Ncat(i);
                dev.Nani(i);];
        end
        u0_ana = u0_ana(1:N_variables);

        % Organise ICs based on number of variables and SOL_IC
        if dficAnalytical
            u0 = u0_ana;
        else
            % Initial conditions taken from input solution
            u0_in = interp1(icx,squeeze(icsol(end,:,:)),x)';
            % If the number of variables has increased then add analytical
            % ICs for missing variables
            if N_variables > length(u0_in)
                % Add initial conditions for new variables from U_ANA
                u0(1:length(u0_in), 1) = u0_in;
                u0(length(u0_in)+1:N_variables, 1) = u0_ana(length(u0_in)+1:N_variables);
            else
                u0 = u0_in;
            end
        end
    end

%% Boundary conditions
% Refer to PDEPE help for the precise meaning of P and Q
% l and r refer to left and right boundaries.
    function [Pl,Ql,Pr,Qr] = dfbc(xl,ul,xr,ur,t)

        switch N_ionic_species
            case 0
                V_l = ul(1);
                V_r = ur(1);
                n_l = ul(2);
                n_r = ur(2);
                p_l = ul(3);
                p_r = ur(3);
                c_l = 0;
                c_r = 0;
                a_l = 0;
                a_r = 0;
            case 1
                V_l = ul(1);
                V_r = ur(1);
                n_l = ul(2);
                n_r = ur(2);
                p_l = ul(3);
                p_r = ur(3);
                c_l = ul(4);
                c_r = ur(4);
                a_l = 0;
                a_r = 0;
            case 2
                V_l = ul(1);
                V_r = ur(1);
                n_l = ul(2);
                n_r = ur(2);
                p_l = ul(3);
                p_r = ur(3);
                c_l = ul(4);
                c_r = ur(4);
                a_l = ul(5);
                a_r = ur(5);
        end

        switch par.V_fun_type
            case 'constant'
                Vapp = par.V_fun_arg(1);
            otherwise
                Vapp = Vapp_fun(par.V_fun_arg, t);
        end

                % Flux boundary conditions for both carrier types.
                % Calculate series resistance voltage Vres
                if Rs == 0
                    Vres = 0;
                else
                    J = e*sp_r*(ur(3) - pright) - e*sn_r*(ur(2) - nright);
                    if Rs_initial
                        Vres = -J*Rs*t/par.tmax;    % Initial linear sweep
                    else
                        Vres = -J*Rs;
                    end
                end

Pl = [-V_l;
  mobset*(-sn_l*(n_l - n0_l));
  mobset*(-sp_l*(p_l - p0_l));
  0;
  0;];

Ql = [0; 1; 1; 1; 1;];

Pr = [-V_r+Vbi-Vapp-Vres;
  mobset*(sn_r*(n_r - n0_r));
  mobset*(sp_r*(p_r - p0_r));
  0;
  0;];

Qr = [0; 1; 1; 1; 1;];


        % Remove unused entries
        Pl = Pl(1:N_variables);
        Pr = Pr(1:N_variables);
        Ql = Ql(1:N_variables);
        Qr = Qr(1:N_variables);
    end
end


==> 2019 Driftfusion methods arXiv submission 2/Lst3_Vapp_function_script.tex <==
% Voltage function type
par.V_fun_type = 'sin';
% DC offset voltage (V)
par.V_fun_arg(1) = 0;
% AC voltage amplitude (V)
par.V_fun_arg(2) = 20e-3;
% Frequency (Hz)
par.V_fun_arg(3) = 1e3;
% Phase (Rads)
par.V_fun_arg(4) = 0;

==> 2019 Driftfusion methods arXiv submission 2/Lst4_doCV.tex <==
function sol_CV = doCV(sol_ini, light_intensity, V0, Vmax, Vmin, scan_rate, cycles, tpoints)
% Performs a cyclic voltammogram (CV) simulation
% Input arguments:
% SOL_INI = solution containing initial conditions
% LIGHT_INTENSITY = Light intensity for bias light (Suns)
% V0 = Starting voltage (V)
% VMAX = Maximum voltage point (V)
% VMIN = Minimum voltage point (V)
% SCAN_RATE = Scan rate (Vs-1)
% CYCLES = No. of scan cycles
% TPOINTS = No. of points in output time array
% P. Calado, 2020, Imperial College London
disp('Starting DOCV')

par = sol_ini.par;

%% Set light intensity
if light_intensity > 0
    sol = lightonRs(sol_ini, light_intensity, -1, 0, 0, 10);
else
    sol = sol_ini;
end

%% Switch to V0 if different from initial conditions
% Trying to do this within the triangular wave function resulted in
% convergence issues so safer to do this here.
if V0 ~= par.Vapp
    sol = genVappStructs(sol, V0, 0);
end

%% Calculate tmax from scan rate and absolute change in voltage, deltaV
deltaV = abs(Vmax-Vmin)+abs(Vmin-Vmax)+abs(V0-Vmin);
tmax = deltaV/scan_rate;

disp('Performing cyclic voltamagram')
sol_CV = VappFunction(sol, 'tri', [V0, Vmax, Vmin, cycles, tmax/cycles], tmax, tpoints, 0);
disp('Complete')

disp('DOCV complete')
end

==> 2019 Driftfusion methods arXiv submission 2/LstS1_pc.tex <==
classdef pc
    % Authors: Philip Calado, Piers Barnes, Ilario Gelmetti, Ben Hillman, 2018 Imperial College London
    % PC (Parameters Class) defines all the required properties for your
    % device. PC.BUILDDEV builds a structure PO.DEV (where PO is a Parameters Object)
    % that defines the properties of the device at every spatial mesh point, including
    % interfaces. Whenever PROPERTIES are overwritten in a protocol, the device should
    % be rebuilt manually using PC.BUILDDEV. The spatial mesh is a linear piece-wise mesh
    % and is built by the MESHGEN_X function. Details of how to define the mesh
    % are given below in the SPATIAL MESH SUBSECTION.

    properties (Constant)
        %% Physical constants
        kB = 8.617330350e-5;     % Boltzmann constant [eV K^-1]
        epp0 = 552434;           % Epsilon_0 [e^2 eV^-1 cm^-1] - Checked (02-11-15)
        q = 1;                   % Charge of the species in units of e.
        e = 1.60217662e-19;         % Elementary charge in Coulombs.
    end

    properties
        % Temperature [K]
        T = 300;

        %% Spatial mesh
        % Device Dimensions [cm]
        % The spatial mesh is a linear piece-wise mesh and is built by the
        % MESHGEN_X function using 2 arrays DCELL and PCELL,
        % which define the thickness and number of points of each layer
        % respectively.
        dcell = 400e-7;         % Layer and subsection thickness array
        layer_points = 400;            % Points array

        %% Layer description
        % Define the layer type for each of the layers in the device. The
        % options are:
        % LAYER = standard layer
        % ACTIVE = standard layer but the properties of this layer are
        % flagged such that they can easily be accessed
        % JUNCTION = a region with graded properties between two materials
        % (either LAYER or ACTIVE type)
        % with different properties
        layer_type = {'active'}
        % STACK is used for reading the optical properties library.
        % The names here do not influence the electrical properties of the
        % device. See INDEX OF REFRACTION LIBRARY for choices- names must be entered
        % exactly as given in the column headings with the '_n', '_k' omitted
        stack = {'MAPICl'}

        % Define spatial cordinate system- typically this will be kept at
        % 0 for most applications
        % m=0 cartesian
        % m=1 cylindrical polar coordinates
        % m=2 spherical polar coordinates
        m = 0;

        %% Spatial mesh
        % xmesh_type specification - see MESHGEN_X.
        xmesh_type = 5;
        xmesh_coeff = [0.7];        % Coefficient array for defining point spacing
        
        %% Time mesh
        % The time mesh is dynamically generated by ODE15s- the mesh
        % defined by MESHGEN_T only defines the values of the points that
        % are read out and so does not influence convergence. Defining an
        % unecessarily high number of points however can be expensive owing
        % to interpolation of the solution.
        tmesh_type = 2;             % Mesh type- for use with meshgen_t
        t0 = 1e-16;                 % Initial log mesh time value
        tmax = 1e-12;               % Max time value
        tpoints = 100;              % Number of time points

        %% GENERAL CONTROL PARAMETERS
        OC = 0;                 % Closed circuit = 0, Open Circuit = 1
        Vapp = 0;               % Applied bias
        BC = 3;                 % Boundary Conditions. Must be set to one for first solution
        figson = 1;             % Toggle figures on/off
        meshx_figon = 0;        % Toggles x-mesh figures on/off
        mesht_figon = 0;        % Toggles t-mesh figures on/off
        side = 1;               % illumination side 1 = left, 2 = right
        calcJ = 0;              % Calculates Currents- slows down solving calcJ = 1, calculates DD currents at every position
        mobset = 1;             % Switch on/off electron hole mobility- MUST BE SET TO ZERO FOR INITIAL SOLUTION
        mobseti = 1;
        SRHset = 1;
        radset = 1;
        JV = 0;                 % Toggle run JV scan on/off
        prob_distro_function = 'Boltz';        % 'Fermi' = Fermi-Dirac, % 'Boltz' = Boltzmann statistics
        Fermi_limit = 0.2;      % Max allowable limit for Fermi levels beyond the bands [eV]
        Fermi_Dn_points = 400;  % No. of points in the Fermi-Dirac look-up table
        intgradfun = 'linear'      % Interface gradient function 'linear' = linear, 'erf' = 'error function'

        %% Generation
        % OM = Optical Model
        % 0 = Uniform Generation
        % 1 = Beer Lambert
        OM = 1;
        Int = 0;                % Bias Light intensity (multiples of g0 or 1 sun for Beer-Lambert)
        int1 = 0;
        int2 = 0;
        g0 = [2.6409e+21];      % Uniform generation rate [cm-3s-1]
        light_source1 = 'AM15';
        light_source2 = 'laser';
        laser_lambda1 = 0;
        laser_lambda2 = 638;
        g1_fun_type = 'constant'
        g2_fun_type = 'constant'
        g1_fun_arg = 0;
        g2_fun_arg = 0;
        % default: Approximate Uniform generation rate @ 1 Sun for 510 nm active layer thickness

        %% Pulse settings
        pulsepow = 10;          % Pulse power [mW cm-2] OM2 (Beer-Lambert and Transfer Matrix only)

        %%%%%%%%%%% LAYER MATERIAL PROPERTIES %%%%%%%%%%%%%%%%%%%%
        % Numerical values should be given as a row vector with the number of
        % entries equal to the number of layers specified in STACK

        %% Energy levels [eV]
        EA = [0];           % Electron affinity
        IP = [-1];           % Ionisation potential

        %% Equilibrium Fermi energies [eV]
        % These define the doping density in each layer- see NA and ND calculations in methods
        E0 = [-0.5];

        %% SRH trap energies [eV]
        % These must exist within the energy gap of the appropriate layers
        % and define the variables PT and NT in the expression:
        % U = (np-ni^2)/(taun(p+pt) +taup(n+nt))
        Et =[-0.5];

        %% Electrode Fermi energies [eV]
        % Fermi energies of the metal electrode. These define the built-in voltage, Vbi
        % and the boundary carrier concentrations nleft, pleft, nright, and
        % pright
        Phi_left = -0.6;
        Phi_right = -0.4;

        %% Effective Density Of States (eDOS) [cm-3]
        Nc = [1e19];
        Nv = [1e19];
        % PEDOT eDOS: https://aip.scitation.org/doi/10.1063/1.4824104
        % MAPI eDOS: F. Brivio, K. T. Butler, A. Walsh and M. van Schilfgaarde, Phys. Rev. B, 2014, 89, 155204.
        % PCBM eDOS:

%% Mobile ions
% Mobile ion defect density [cm-3]
N_ionic_species = 1;
K_anion = 1;         % Coefficients to easily accelerate ions
K_cation = 1;        % Coefficients to easily accelerate ions
Nani = [1e19];
Ncat = [1e19];
% Approximate density of iodide sites [cm-3]
% Limits the density of iodide vancancies
a_max = [1.21e22];
c_max = [1.21e22]; 
% Ionic generation and recombination rates
k_iongen = [0];
k_ionrec = [0];
        
%% Mobilities   [cm2V-1s-1]
mu_n = [1];         % electron mobility
mu_p = [1];         % hole mobility

mu_a = [1e-10];          % ion mobility
mu_c = [1e-14];
        

        
        % PTPD h+ mobility: https://pubs.rsc.org/en/content/articlehtml/2014/ra/c4ra05564k
        % PEDOT mue = 0.01 cm2V-1s-1 https://aip.scitation.org/doi/10.1063/1.4824104
        % TiO2 mue = 0.09 cm2V-1s-1 Bak2008
        % Spiro muh = 0.02 cm2V-1s-1 Hawash2018

        %% Relative dielectric constants
        epp = [10];

        %% Recombination
        % Radiative recombination, U = k(np - ni^2)
        % [cm3 s-1] Radiative Recombination coefficient
        krad = [3.6e-12];

        %% SRH time constants for each layer [s]
        taun = [1e6];           % [s] SRH time constant for electrons
        taup = [1e6];           % [s] SRH time constant for holes

        %% Surface recombination and extraction coefficients [cm s-1]
        % Descriptions given in the comments considering that holes are
        % extracted at left boundary, electrons at right boundary
        sn_l = 1e7;     % electron surface recombination velocity left boundary
        sn_r = 1e7;     % electron extraction velocity right boundary
        sp_l = 1e7;     % hole extraction left boundary
        sp_r = 1e7;     % hole surface recombination velocity right boundary

        %% Series resistance
        Rs = 0;
        Rs_initial = 0;         % Switch to allow linear ramp of Rs on first application

        %% Dynamically created variables
        genspace = [];
        x = [];
        xx = [];
        x_ihalf = [];
        dev = [];
        dev_ihalf = [];
        t = [];
        xpoints = [];
        gx1 = [];       % Light source 1
        gx2 = [];       % Light source 2

        %% Voltage function parameters
        V_fun_type = 'constant';
        V_fun_arg = 0;
        
        % Define the default relative tolerance for the pdepe solver
        % 1e-3 is the default, can be decreased if more precision is needed
        % Solver options
        MaxStepFactor = 1;      % Multiplier for easy access to maximum time step
        RelTol = 1e-3;
        AbsTol = 1e-6;
        
        %% Impedance parameters
        J_E_func = [];
        J_E_func_tilted = [];
        E2_func = [];
    end

    %%  Properties whose values depend on other properties (see 'get' methods).
    properties (Dependent)
        active_layer
        d
        parr
        d_active
        dcum
        dcum0           % includes first entry as zero
        d_midactive
        dEAdx
        dIPdx
        dNcdx
        dNvdx
        Dn
        Eg
        Eif
        NA
        ND
        Vbi
        n0
        nleft
        nright
        ni
        nt_bulk         % Density of CB electrons when Fermi level at trap state energy
        nt_inter
        p0
        pcum
        pcum0           % Includes first entry as zero
        pleft
        pright
        pt_bulk         % Density of VB holes when Fermi level at trap state energy
        pt_inter
        wn
        wp
        wscr            % Space charge region width
        x0              % Initial spatial mesh value

    end

    methods
        function par = pc(varargin)
            % Parameters constructor function- runs numerous checks that
            % the input properties are consistent with the model
            if length(varargin) == 1
                % Use argument as filepath and overwrite properties using
                % PC.IMPORTPROPERTIES
                filepath = varargin;
                par = import_properties(par, filepath);
            elseif length(varargin) > 1
                filepath = varargin{1, 1};
                warning('pc should have 0 or 1 input arguments- only the first argument will be used for the filepath')
            end

            % Warn if tmesh_type is not correct
            if ~ any([1 2 3 4] == par.tmesh_type)
                warning('PARAMS.tmesh_type should be an integer from 1 to 3 inclusive. MESHGEN_T cannot generate a mesh if this is not the case.')
            end

            % Warn if xmesh_type is not correct
            if ~ any(1:1:5 == par.xmesh_type)
                warning('PARAMS.xmesh_type should be an integer from 1 to 5 inclusive. MESHGEN_X cannot generate a mesh if this is not the case.')
            end

            % Warn if doping density exceeds eDOS
            for i = 1:length(par.ND)
                if par.ND(i) > par.Nc(i) || par.NA(i) > par.Nc(i)
                    msg = 'Doping density must be less than eDOS. For consistent values ensure electrode workfunctions are within the band gap and check expressions for doping density in Dependent variables.';
                    error(msg);
                end
            end

            % Warn if trap energies are outside of band gap energies
            for i = 1:length(par.Et)
                if par.Et(i) >= par.EA(i) || par.Et(i) <= par.IP(i)
                    msg = 'Trap energies must exist within layer band gap.';
                    error(msg);
                end
            end

            % Warn if DOSani is set to zero in any layers - leads to
            % infinite diffusion rate
            for i = 1:length(par.DOSani)
                if par.DOSani(i) <= 0
                    msg = 'ion DOS (DOSani) cannot have zero or negative entries- choose a low value rather than zero e.g. 1';
                    error(msg);
                end
            end

            % Warn if electrode workfunctions are outside of boundary layer
            % bandgap
            if par.Phi_left < par.IP(1) || par.Phi_left > par.EA(1)
                msg = 'Left-hand workfunction (Phi_left) out of range: value must exist within left-hand layer band gap';
                error(msg)
            end

            if par.Phi_right < par.IP(end) || par.Phi_right > par.EA(end)
                msg = 'Right-hand workfunction (Phi_right) out of range: value must exist within right-hand layer band gap';
                error(msg)
            end

            % Warn if property array do not have the correct number of
            % layers. The layer thickness array is used to define the
            % number of layers
            if length(par.parr) ~= length(par.d)
                msg = 'Points array (parr) does not have the correct number of elements. Property arrays must have the same number of elements as the thickness array (d), except SRH properties for interfaces which should have length(d)-1 elements.';
                error(msg);
            elseif length(par.EA) ~= length(par.d)
                msg = 'Electron Affinity array (EA) does not have the correct number of elements. Property arrays must have the same number of elements as the thickness array (d), except SRH properties for interfaces which should have length(d)-1 elements.';
                error(msg);
            elseif length(par.IP) ~= length(par.d)
                msg = 'Ionisation Potential array (IP) does not have the correct number of elements. Property arrays must have the same number of elements as the thickness array (d), except SRH properties for interfaces which should have length(d)-1 elements.';
                error(msg);
            elseif length(par.mue) ~= length(par.d)
                msg = 'Electron mobility array (mue) does not have the correct number of elements. Property arrays must have the same number of elements as the thickness array (d), except SRH properties for interfaces which should have length(d)-1 elements.';
                error(msg);
            elseif length(par.muh) ~= length(par.d)
                msg = 'Hole mobility array (mue) does not have the correct number of elements. Property arrays must have the same number of elements as the thickness array (d), except SRH properties for interfaces which should have length(d)-1 elements.';
                error(msg);
            elseif length(par.muani) ~= length(par.d)
                msg = 'Ion mobility array (muh) does not have the correct number of elements. Property arrays must have the same number of elements as the thickness array (d), except SRH properties for interfaces which should have length(d)-1 elements.';
                error(msg);
            elseif length(par.NA) ~= length(par.d)
                msg = 'Acceptor density array (NA) does not have the correct number of elements. Property arrays must have the same number of elements as the thickness array (d), except SRH properties for interfaces which should have length(d)-1 elements.';
                error(msg);
            elseif length(par.ND) ~= length(par.d)
                msg = 'Donor density array (ND) does not have the correct number of elements. Property arrays must have the same number of elements as the thickness array (d), except SRH properties for interfaces which should have length(d)-1 elements.';
                error(msg);
            elseif length(par.Nc) ~= length(par.d)
                msg = 'Effective density of states array (Nc) does not have the correct number of elements. Property arrays must have the same number of elements as the thickness array (d), except SRH properties for interfaces which should have length(d)-1 elements.';
                error(msg);
            elseif length(par.Nv) ~= length(par.d)
                msg = 'Effective density of states array (Nv) does not have the correct number of elements. Property arrays must have the same number of elements as the thickness array (d), except SRH properties for interfaces which should have length(d)-1 elements.';
                error(msg);
            elseif length(par.Nani) ~= length(par.d)
                msg = 'Background ion density (Nani) does not have the correct number of elements. Property arrays must have the same number of elements as the thickness array (d), except SRH properties for interfaces which should have length(d)-1 elements.';
                error(msg);
            elseif length(par.DOSani) ~= length(par.d)
                msg = 'Ion density of states array (DOSani) does not have the correct number of elements. Property arrays must have the same number of elements as the thickness array (d), except SRH properties for interfaces which should have length(d)-1 elements.';
                error(msg);
            elseif length(par.epp) ~= length(par.d)
                msg = 'Relative dielectric constant array (epp) does not have the correct number of elements. Property arrays must have the same number of elements as the thickness array (d), except SRH properties for interfaces which should have length(d)-1 elements.';
                error(msg);
            elseif length(par.krad) ~= length(par.d)
                msg = 'Radiative recombination coefficient array (krad) does not have the correct number of elements. Property arrays must have the same number of elements as the thickness array (d), except SRH properties for interfaces which should have length(d)-1 elements.';
                error(msg);
            elseif length(par.E0) ~= length(par.d)
                msg = 'Equilibrium Fermi level array (E0) does not have the correct number of elements. Property arrays must have the same number of elements as the thickness array (d), except SRH properties for interfaces which should have length(d)-1 elements.';
                error(msg);
            elseif length(par.g0) ~= length(par.d)
                msg = 'Uniform generation array (g0) does not have the correct number of elements. Property arrays must have the same number of elements as the thickness array (d), except SRH properties for interfaces which should have length(d)-1 elements.';
                error(msg);
            elseif length(par.taun) ~= length(par.d)
                msg = 'Bulk SRH electron time constants array (taun_bulk) does not have the correct number of elements. Property arrays must have the same number of elements as the thickness array (d), except SRH properties for interfaces which should have length(d)-1 elements.';
                error(msg);
            elseif length(par.taup) ~= length(par.d)
                msg = 'Bulk SRH hole time constants array (taup_bulk) does not have the correct number of elements. Property arrays must have the same number of elements as the thickness array (d), except SRH properties for interfaces which should have length(d)-1 elements.';
                error(msg);
            elseif length(par.Et) ~= length(par.d)
                msg = 'Bulk SRH trap energy array (Et) does not have the correct number of elements. Property arrays must have the same number of elements as the thickness array (d), except SRH properties for interfaces which should have length(d)-1 elements.';
                error(msg);
            end

            %% Device and generation builder
            % Import variables and structure, xx, gx1, gx2, and dev must be
            % refreshed when to rebuild the device for example when
            % changing device thickness on the fly. These are not present
            % in the dependent variables as it is too costly to have them
            % continuously called.
            par = refresh_device(par);
        end

        function par = set.xmesh_type(par, value)
            %   SET.xmesh_type(PARAMS, VALUE) checks if VALUE is an integer
            %   from 1 to 3, and if so, changes PARAMS.xmesh_type to VALUE.
            %   Otherwise, a warning is shown. Runs automatically whenever
            %   xmesh_type is changed.
            if any(1:1:5 == value)
                par.xmesh_type = value;
            else
                error('PARAMS.xmesh_type should be an integer from 1 to 3 inclusive. MESHGEN_X cannot generate a mesh if this is not the case.')
            end
        end

        function par = set.tmesh_type(par, value)
            %   SET.tmesh_type(PARAMS, VALUE) checks if VALUE is an integer
            %   from 1 to 2, and if so, changes PARAMS.tmesh_type to VALUE.
            %   Otherwise, a warning is shown. Runs automatically whenever
            %   tmesh_type is changed.
            if any(1:1:4 == value)
                par.tmesh_type = value;
            else
                error('PARAMS.tmesh_type should be an integer from 1 to 4 inclusive. MESHGEN_T cannot generate a mesh if this is not the case.')
            end
        end

        function par = set.ND(par, value)
            for i = 1:length(par.ND)
                if value(i) >= par.Nc(i)
                    error('Doping density must be less than eDOS. For consistent values ensure electrode workfunctions are within the band gap.')
                end
            end
        end

        function par = set.NA(par, value)
            for i = 1:length(par.ND)
                if value(i) >= par.Nv(i)
                    error('Doping density must be less than eDOS. For consistent values ensure electrode workfunctions are within the band gap.')
                end
            end
        end

        %% Get active layer indexes from layer_type
        function value = get.active_layer(par)
            value = find(strncmp('active', par.layer_type,6));
            if length(value) == 0
                % If no flag is give assume active layer is middle
                value = round(length(par.layer_type)/2);
            end
        end

        %% Active layer thickness
        function value = get.d_active(par)
            value = sum(par.dcell(par.active_layer(1):par.active_layer(end)));
        end
    
        function value = get.d_midactive(par)
           value = par.dcum(par.active_layer(1)-1) + par.d_active/2;
        end
        %% Layer thicknesses [cm]
        function value = get.d(par)
            % For backwards comptibility. layer_points and parr arre the now the
            % same thing
            value = par.dcell;
        end

        %% Layer points
        function value = get.parr(par)
            % For backwards comptibility. layer_points and parr arre the now the
            % same thing
            value = par.layer_points;
        end

        %% Band gap energies    [eV]
        function value = get.Eg(par)
            value = par.EA - par.IP;
        end

        %% Built-in voltage Vbi based on difference in boundary workfunctions
        function value = get.Vbi(par)
            value = par.Phi_right - par.Phi_left;
        end

        %% Intrinsic Fermi Energies
        % Currently uses Boltzmann stats as approximation should always be
        function value = get.Eif(par)
            value = 0.5.*(par.EA+par.IP)+par.kB*par.T*log(par.Nc./par.Nv);
        end

        %% Donor densities
        function value = get.ND(par)
            value = zeros(1, length(par.stack));
            value = distro_fun.nfun(par.Nc, par.EA, par.E0, par.T, par.prob_distro_function);
        end

        %% Acceptor densities
        function value = get.NA(par)
            value = zeros(1, length(par.stack));
            value = distro_fun.pfun(par.Nv, par.IP, par.E0, par.T, par.prob_distro_function);
        end

        %% Intrinsic carrier densities (Boltzmann)
        function value = get.ni(par)
            value = par.Nc.*exp(-par.Eg./(2*par.kB*par.T));
        end

        %% Equilibrium electron densities
        function value = get.n0(par)
            value = distro_fun.nfun(par.Nc, par.EA, par.E0, par.T, par.prob_distro_function);
        end

        %% Equilibrium hole densities
        function value = get.p0(par)
            value = distro_fun.pfun(par.Nv, par.IP, par.E0, par.T, par.prob_distro_function);

        end

        %% Boundary electron and hole densities
        % Uses metal Fermi energies to calculate boundary densities
        % Electrons left boundary
        function value = get.nleft(par)
            value = distro_fun.nfun(par.Nc(1), par.EA(1), par.Phi_left, par.T, par.prob_distro_function);
        end

        % Electrons right boundary
        function value = get.nright(par)
            value = distro_fun.nfun(par.Nc(end), par.EA(end), par.Phi_right, par.T, par.prob_distro_function);
        end

        % Holes left boundary
        function value = get.pleft(par)
            value = distro_fun.pfun(par.Nv(1), par.IP(1), par.Phi_left, par.T, par.prob_distro_function);
        end

        % holes right boundary
        function value = get.pright(par)
            value = distro_fun.pfun(par.Nv(end), par.IP(end), par.Phi_right, par.T, par.prob_distro_function);
        end

        function value = get.dcum(par)
            value = cumsum(par.dcell);
        end

        function value = get.pcum(par)
            value = cumsum(par.layer_points);
        end

        function value = get.pcum0(par)
            value = [1, cumsum(par.layer_points)];
        end

        function value = get.dcum0(par)
            value = [0, cumsum(par.dcell)];
        end
    end

    methods (Static)

        function xx = xmeshini(par) % For backwards compatibility
            xx = meshgen_x(par);
        end     

    end
end


==> 2019 Driftfusion methods arXiv submission 2/LstS3_import_properties.tex <==
function par = import_properties(par, filepath)
% A function to IMPORT_PROPERTIES from a text file LOCATED at FILEPATH. Each of the listed properties
% is checked to see if it is available in the .CSV file. If it is available, the existing properties
% are overwritten otherwise a warning is displayed.

T = readtable(filepath{1,1});   % Reads-in in the external .CSV file to a table T

try
    par.layer_type = T{:,'layer_type'}';
catch
    warning('No layer type (layer_type) defined in .csv . Using default in PC')
end
try
    par.stack = T{:,'stack'}';
catch
    warning('No stack (stack) defined in .csv . Using default in PC')
end
try
    par.dcell = T{:, 'thickness'}';
catch
    warning('No thickness array (thickness) defined in .csv . Using default in PC')
end
try
    par.layer_points = T{:, 'layer_points'}';
catch
    warning('No layer points array (points) defined in .csv . Using default in PC')
end
try
    par.xmesh_coeff = T{:, 'xmesh_coeff'}';
catch
    warning('No xmesh coefficient array (xmesh_coeff) defined in .csv . Using default in PC')
end
try
    par.EA = T{:, 'EA'}';
catch
    warning('No electron affinity array (EA) defined in .csv . Using default in PC')
end
try
    par.IP = T{:, 'IP'}';
catch
    warning('No ionisation potential array (IP) defined in .csv . Using default in PC')
end
try
    par.E0 = T{:, 'E0'}';
catch
    warning('No equilibrium Fermi level array (E0) defined in .csv . Using default in PC')
end
try
    par.Nc = T{:, 'Nc'}';
catch
    warning('No conduction band eDOS array (Nc) defined in .csv . Using default in PC')
end
try
    par.Nv = T{:, 'Nv'}';
catch
    warning('No valence band eDOS array (Nv) defined in .csv . Using default in PC')
end
try
    par.Nani = T{:, 'Nani'}';
catch
    warning('No equilibrium anion density array (Nani) defined in .csv . Using default in PC')
end
try
    par.Ncat = T{:, 'Ncat'}';
catch
    warning('No equilibrium cation density array (Ncat) defined in .csv . Using default in PC')
end
try
    par.DOSani = T{:, 'DOSani'}';
catch
    warning('No maximum anion density array (DOSani) defined in .csv . Using default in PC')
end
try
    par.DOScat = T{:, 'DOScat'}';
catch
    warning('No maximum cation density array (DOScat) defined in .csv . Using default in PC')
end
try
    par.mue = T{:, 'mue'}';
catch
    warning('No electron mobility (mue) defined in .csv . Using default in PC')
end
try
    par.muh = T{:, 'muh'}';
catch
    warning('No hole mobility (muh) defined in .csv . Using default in PC')
end

try
    par.muani = T{:, 'muani'}';
catch
    warning('No anion mobility (muani) defined in .csv . Using default in PC')
end
try
    par.mucat = T{:, 'mucat'}';
catch
    warning('No cation mobility (mucat) defined in .csv . Using default in PC')
end
try
    par.epp = T{:, 'epp'}';
catch
    warning('No relative dielectric constant (epp) defined in .csv . Using default in PC')
end

try
    par.g0 = T{:, 'g0'}';
catch
    warning('No uniform generation rate (g0) defined in .csv . Using default in PC')
end
try
    par.krad = T{:, 'krad'}';
catch
    warning('No radiative recombinaiton coefficient array (krad) defined in .csv . Using default in PC')
end

try
    par.taun = T{:, 'taun'}';
catch
    warning('No SRH electron lifetime array (taun) defined in .csv . Using default in PC')
end
try
    par.taup = T{:, 'taup'}';
catch
    warning('No SRH hole lifetime array (taup) defined in .csv . Using default in PC')
end
try
    par.sn_l = T{1, 'sn_l'}';
catch
    warning('No sn_l defined in .csv . Using default in PC')
end
try
    par.sp_l = T{1, 'sp_l'}';
catch
    warning('No sp_l defined in .csv . Using default in PC')
end
try
    par.sn_r = T{1, 'sn_r'}';
catch
    warning('No sn_r defined in .csv . Using default in PC')
end
try
    par.sp_r = T{1, 'sp_r'}';
catch
    warning('No sp_r defined in .csv . Using default in PC')
end

try
    par.Phi_left = T{1, 'Phi_left'};
catch
    warning('No Phi_left defined in .csv . Using default in PC')
end
try
    par.Phi_right = T{1, 'Phi_right'};
catch
    warning('No Phi_right defined in .csv . Using default in PC')
end
try
    par.Et = T{:,'Et'}';
catch
    warning('No trap energy array (Et) defined in .csv . Using default in PC')
end
try
    par.OM = T{1, 'OM'};
catch
    warning('No optical model (OM) specified in .csv Using default in PC')
end
try
    par.xmesh_type = T{1, 'xmesh_type'};
catch
    warning('No spatial mesh type (xmesh_type) defined in .csv . Using default in PC')
end
try
    par.side = T{1, 'side'};
catch
    warning('Illumination side (side) undefined in .csv . Using default in PC')
end
try
    par.N_ionic_species = T{1, 'N_ionic_species'};
catch
    warning('No of ionic species (N_ionic_species) undefined in .csv. Using default in PC')
end
try
    par.k_iongen = T{1, 'k_iongen'};
catch
    warning('k_iongen undefined in .csv. Using default in PC')
end
try
    par.k_ionrec = T{1, 'k_ionrec'};
catch
    warning('k_ionrec undefined in .csv. Using default in PC')
end

%% Additional checks for backwards compatibility- old variable names
% No warning required otherwise will constantly warn when building
% parameters object
try
    par.Nani = T{:, 'Nion'}';
end
try
    par.DOSani = T{:, 'DOSion'}';
end
try
    par.muani = T{:, 'muion'}';
end
try
    par.Et = T{:,'Et_bulk'}';
end
try
    par.taun = T{:, 'taun_SRH'}';
end
try
    par.taup = T{:, 'taup_SRH'}';
end
try
    par.g0 = T{:, 'G0'}';
end
try
    par.Phi_left = T{1, 'PhiA'};
end
try
    par.Phi_right = T{1, 'PhiC'}; 
end
try
    par.layer_points = T{:, 'points'}';
end
end

==> 2019 Driftfusion methods arXiv submission 2/LstS4_df_ion_gen.tex <==
function solstruct = df(varargin)
% Core DRIFTFUSION function- organises properties and inputs for pdepe
% A routine to test solving the diffusion and drift equations using the
% matlab pepde solver.
%
%% LICENSE
% Copyright (C) 2020  Philip Calado, Ilario Gelmetti, and Piers R. F. Barnes
% Imperial College London
% This program is free software: you can redistribute it and/or modify
% it under the terms of the GNU Affero General Public License as published
% by the Free Software Foundation, either version 3 of the License, or
% (at your option) any later version.
%
% Solution outputs
% V = u(1) = electrostatic potential
% n = u(2) = electron density
% p = u(3) = holes density
% c = u(4) = cation density (optional)
% a = u(5) = anion density (optional)
%
%% Start code
%% Deal with input arguments
if length(varargin) == 0
    % If no input parameter set then call pc directly
    par = pc;
    dficAnalytical = true;
elseif length(varargin) == 1
    % If one input argument then assume it is the Initial Conditions (IC) solution
    icsol = varargin{1, 1}.u;
    icx = varargin{1, 1}.x;
    par = varargin{1, 1}.par;
    dficAnalytical = false;
elseif length(varargin) == 2
    if max(max(max(varargin{1, 1}.u))) == 0
        par = varargin{2};
        dficAnalytical = true;
    elseif isa(varargin{2}, 'char') == 1            % Checks to see if argument is a character
        input_solstruct = varargin{1, 1};
        par = input_solstruct.par;
        icsol = input_solstruct.u;
        icx = input_solstruct.x;
        dficAnalytical = false;
    else
        input_solstruct = varargin{1, 1};
        icsol = input_solstruct.u;
        icx = input_solstruct.x;
        par = varargin{2};
        dficAnalytical = false;
    end
end

%% Unpack properties
%% Spatial mesh
xmesh = par.xx;
x_sub = par.x_sub;
x = xmesh;

%% Time mesh
t = meshgen_t(par);

%% Dependent properties: Prevents recalculation of dependent properties by pdepe defined in Methods
% Can also use AbortSet in class def
Vbi = par.Vbi;
nleft = par.nleft;
nright = par.nright;
pleft = par.pleft;
pright = par.pright;
dev = par.dev;

%% Constants
kB = par.kB;
q = par.q;
e = par.e;
epp0 = par.epp0;

%% Device parameters
device = par.dev_sub;
T = par.T;
mue = device.mue;           % Electron mobility
muh = device.muh;           % Hole mobility
Dn = mue*kB*T;              % Electron diffusion coefficient
Dp = muh*kB*T;              % Hole diffusion coefficient
mucat = device.mucat;       % Cation mobility
muani = device.muani;       % Anion mobility
Nc = device.Nc;             % Conduction band effective density of states
Nv = device.Nv;             % Valence band effective density of states
cmax = device.cmax;     % Cation density upper limit
amax = device.amax;     % Anion density upper limit
gradNc = device.gradNc;     % Conduction band effective density of states gradient
gradNv = device.gradNv;     % Valence band effective density of states gradient
gradEA = device.gradEA;     % Electron Affinity gradient
gradIP = device.gradIP;     % Ionisation Potential gradient
epp = device.epp;           % Dielectric constant
eppmax = max(par.epp);      % Maximum dielectric constant (for normalisation)
B = device.B;               % Radiative recombination rate coefficient
ni = device.ni;             % Intrinsic carrier density
taun = device.taun;         % Electron SRH time constant
taup = device.taup;         % Electron SRH time constant
taun_vsr = device.taun_vsr; % Electron SRH time constant- volumetric interfacial surface recombination scheme
taup_vsr = device.taup_vsr; % Electron SRH time constant- volumetric interfacial surface recombination scheme
k_iongen = device.k_iongen; % Ion generation coefficient
k_ionrec = device.k_ionrec; % Ion recombination coefficient
nt = device.nt;             % SRH electron trap constant
pt = device.pt;             % SRH hole trap constant
NA = device.NA;             % Acceptor doping density
ND = device.ND;             % Donor doping density
Ncat = device.Ncat;         % Uniform cation density
Nani = device.Nani;         % Uniform anion density
xprime_n = device.xprime_n;         % Translated x co-ordinates for interfaces
xprime_p = device.xprime_p;         % Translated x co-ordinates for interfaces
sign_xn = device.sign_xn;           % 1 if xn increasing, -1 if decreasing wrt x
sign_xp = device.sign_xp;           % 1 if xp increasing, -1 if decreasing wrt x
alpha0_xn = device.alpha0_xn;       % alpha0_xn is alpha for F = 0 reference to xprime_n
beta0_xp = device.beta0_xp;         % beta0_xp is beta for F = 0 referenced to xprime_p
N_max_variables = par.N_max_variables;  % Maximum number of variables allowable in this version of Driftfusion
N_ionic_species = par.N_ionic_species;  % Number of ionic species in this solution
N_variables = par.N_ionic_species + 3;  % Number of variables in this solution (+3 for V, n, and p)

z_c = par.z_c;
z_a = par.z_a;
nleft = par.nleft;
nright = par.nright;
pleft = par.pleft;
pright = par.pright;
sn_l = par.sn_l;
sp_l = par.sp_l;
sn_r = par.sn_r;
sp_r = par.sp_r;
Rs = par.Rs;
Rs_initial = par.Rs_initial;

%% Switches and accelerator coefficients
mobset = par.mobset;        % Electronic carrier transport switch
mobseti = par.mobseti;      % Ionic carrier transport switch
K_cation = par.K_cation;    % Cation transport rate multiplier
K_anion = par.K_anion;      % Anion transport rate multiplier
radset = par.radset;        % Radiative recombination switch
SRHset = par.SRHset;        % SRH recombination switch
vsr_zone = device.vsr_zone;

%% Generation
g1_fun = fun_gen(par.g1_fun_type);
g2_fun = fun_gen(par.g2_fun_type);
gxt1 = 0;
gxt2 = 0;
g = 0;
gx1 = par.gx1;
gx2 = par.gx2;
int1 = par.int1;
int2 = par.int2;
g1_fun_type = par.g1_fun_type;
g2_fun_type = par.g2_fun_type;
g1_fun_arg = par.g1_fun_arg;
g2_fun_arg = par.g2_fun_arg;

%% Voltage function
Vapp_fun = fun_gen(par.V_fun_type);
Vapp = 0;
Vres = 0;
J = 0;

%% Solver variables
V = 0; n = 0; p = 0; a = 0; c = 0;
dVdx = 0; dndx = 0; dpdx = 0; dadx = 0; dcdx = 0;
C_V = 0; C_n = 0; C_p = 0; C_c = 0; C_a = 0;
F_V = 0; F_n = 0; F_p = 0; F_c = 0; F_a = 0;
S_V = 0; S_n = 0; S_p = 0; S_c = 0; S_a = 0;
r_rad = 0; r_srh = 0; r_vsr = 0; r_np = 0;
alpha = 0; beta = 0;

%% Solver options
% MaxStep = limit maximum time step size during integration
options = odeset('MaxStep', par.MaxStepFactor*0.1*abs(par.tmax - par.t0), 'RelTol', par.RelTol, 'AbsTol', par.AbsTol, 'NonNegative', [1,1,1,0]);

%% Call solver
% inputs with '@' are function handles to the subfunctions
% below for the: equation, initial conditions, boundary conditions
u = pdepe(par.m,@dfpde,@dfic,@dfbc,x,t,options);

%% Ouputs
% Store final voltage reading
par.Vapp = Vapp;

% Solutions and meshes to structure
solstruct.u = u;
solstruct.x = x;
solstruct.t = t;

% Store parameters object
solstruct.par = par;

%% Volumetric surface recombination error check
if par.vsr_mode == 1 && par.vsr_check == 1
    compare_rec_flux(solstruct, par.RelTol_vsr, par.AbsTol_vsr, 0);
end

%% Subfunctions
% Set up partial differential equation (pdepe) (see MATLAB pdepe help for details of C,F,S)
% C = Time-dependence prefactor
% F = Flux terms
% S = Source terms
    function [C,F,S] = dfpde(x,t,u,dudx)
        % Get position point
        i = find(x_sub <= x);
        i = i(end);

        switch g1_fun_type
            case 'constant'
                gxt1 = int1*gx1(i);
            otherwise
                gxt1 = g1_fun(g1_fun_arg, t)*gx1(i);
        end

        switch g2_fun_type
            case 'constant'
                gxt2 = int2*gx2(i);
            otherwise
                gxt2 = g2_fun(g2_fun_arg, t)*gx2(i);
        end
        g = gxt1 + gxt2;

        %% Unpack Variables
        
        
                V = u(1);
                n = u(2);
                p = u(3);
                c = u(4);
                a = u(5);
                dVdx = dudx(1);
                dndx = dudx(2);
                dpdx = dudx(3);
                dcdx = dudx(4);
                dadx = dudx(5);












%% Equation editor
% Time-dependence prefactor term
C_V = 0; C_n = 1; C_p = 1; C_c = 1; C_a = 1;
C = [C_V; C_n; C_p; C_c; C_a];

% Flux terms
F_V = (epp(i)/eppmax)*dVdx;
F_n = mu_n(i)*n*(-dVdx + gradEA(i)) + (Dn(i)*(dndx - ((n/Nc(i))*gradNc(i))));
F_p = mu_p(i)*p*(dVdx - gradIP(i)) + (Dp(i)*(dpdx - ((p/Nv(i))*gradNv(i))));
F_c = mu_c(i)*(z_c*c*dVdx + kB*T*(dcdx + (c*(dcdx/(c_max(i) - c)))));
F_a = mu_a(i)*(z_a*a*dVdx + kB*T*(dadx + (a*(dadx/(a_max(i) - a)))));
F = [F_V; mobset*F_n; mobset*F_p; mobseti*K_c*F_c; mobseti*K_a*F_a];

% Electron and hole recombination
% Radiative
r_rad = radset*B(i)*(n*p - ni(i)^2);
% Bulk SRH
r_srh = SRHset*srh_zone(i)*((n*p - ni(i)^2)/(taun(i)*(p + pt(i)) + taup(i)*(n + nt(i))));
% Volumetric surface recombination
alpha = sign_xn(i)*q*dVdx/(kB*T) + alpha0_xn(i);
beta = sign_xp(i)*q*-dVdx/(kB*T) + beta0_xp(i);
r_vsr = SRHset*vsr_zone(i)*((n*exp(-alpha*xprime_n(i))*p*exp(-beta*xprime_p(i)) - ni(i)^2)...
    /(taun_vsr(i)*(p*exp(-beta*xprime_p(i)) + pt(i)) + taup_vsr(i)*(n*exp(-alpha*xprime_n(i)) + nt(i))));
% Total electron and hole recombination
r_np = r_rad + r_srh + r_vsr;

% Source terms
S_V = (q/(eppmax*epp0))*(-n + p - NA(i) + ND(i) + z_a*a + z_c*c - z_a*Nani(i) - z_c*Ncat(i));
S_n = g - r_np;
S_p = g - r_np;
S_c = k_iongen*g - k_ionrec*(c*a-Ncat(i)*Nani(i));
S_a = 0;
S = [S_V; S_n; S_p; S_c; S_a];

        % Remove unused variables - faster and tidier than using conditional
        % statements
        C = C(1:N_variables);
        F = F(1:N_variables);
        S = S(1:N_variables);
    end

%% Initial conditions.
    function u0 = dfic(x)
        i = find(xmesh <= x);
        i = i(end);

        if length(par.dcell) == 1
            % Single layer
            u0_ana = [(x/xmesh(end))*Vbi;
                nleft*exp((x*(log(nright)-log(nleft)))/par.dcum0(end));
                pleft*exp((x*(log(pright)-log(pleft)))/par.dcum0(end));
                dev.Ncat(i);
                dev.Nani(i);];
        else
            % Multi-layered
            u0_ana = [(x/xmesh(end))*Vbi;
                dev.n0(i);
                dev.p0(i);
                dev.Ncat(i);
                dev.Nani(i);];
        end
        u0_ana = u0_ana(1:N_variables);

        % Organise ICs based on number of variables and SOL_IC
        if dficAnalytical
            u0 = u0_ana;
        else
            % Initial conditions taken from input solution
            u0_in = interp1(icx,squeeze(icsol(end,:,:)),x)';
            % If the number of variables has increased then add analytical
            % ICs for missing variables
            if N_variables > length(u0_in)
                % Add initial conditions for new variables from U_ANA
                u0(1:length(u0_in), 1) = u0_in;
                u0(length(u0_in)+1:N_variables, 1) = u0_ana(length(u0_in)+1:N_variables);
            else
                u0 = u0_in;
            end
        end
    end

%% Boundary conditions
% Refer to PDEPE help for the precise meaning of P and Q
% l and r refer to left and right boundaries.
    function [Pl,Ql,Pr,Qr] = dfbc(xl,ul,xr,ur,t)

        switch N_ionic_species
            case 0
                V_l = ul(1);
                V_r = ur(1);
                n_l = ul(2);
                n_r = ur(2);
                p_l = ul(3);
                p_r = ur(3);
                c_l = 0;
                c_r = 0;
                a_l = 0;
                a_r = 0;
            case 1
                V_l = ul(1);
                V_r = ur(1);
                n_l = ul(2);
                n_r = ur(2);
                p_l = ul(3);
                p_r = ur(3);
                c_l = ul(4);
                c_r = ur(4);
                a_l = 0;
                a_r = 0;
            case 2
                V_l = ul(1);
                V_r = ur(1);
                n_l = ul(2);
                n_r = ur(2);
                p_l = ul(3);
                p_r = ur(3);
                c_l = ul(4);
                c_r = ur(4);
                a_l = ul(5);
                a_r = ur(5);
        end

        switch par.V_fun_type
            case 'constant'
                Vapp = par.V_fun_arg(1);
            otherwise
                Vapp = Vapp_fun(par.V_fun_arg, t);
        end

                % Flux boundary conditions for both carrier types.
                % Calculate series resistance voltage Vres
                if Rs == 0
                    Vres = 0;
                else
                    J = e*sp_r*(ur(3) - pright) - e*sn_r*(ur(2) - nright);
                    if Rs_initial
                        Vres = -J*Rs*t/par.tmax;    % Initial linear sweep
                    else
                        Vres = -J*Rs;
                    end
                end

Pl = [-V_l;
  mobset*(-sn_l*(n_l - n0_l));
  mobset*(-sp_l*(p_l - p0_l));
  0;
  0;];

Ql = [0; 1; 1; 1; 1;];

Pr = [-V_r+Vbi-Vapp-Vres;
  mobset*(sn_r*(n_r - n0_r));
  mobset*(sp_r*(p_r - p0_r));
  0;
  0;];

Qr = [0; 1; 1; 1; 1;];


        % Remove unused entries
        Pl = Pl(1:N_variables);
        Pr = Pr(1:N_variables);
        Ql = Ql(1:N_variables);
        Qr = Qr(1:N_variables);
    end
end


==> Lst1_Equation_editor.tex <==
function solstruct = df(varargin)
% Core DRIFTFUSION function- organises properties and inputs for pdepe
% A routine to test solving the diffusion and drift equations using the
% matlab pepde solver.
%
%% LICENSE
% Copyright (C) 2020  Philip Calado, Ilario Gelmetti, and Piers R. F. Barnes
% Imperial College London
% This program is free software: you can redistribute it and/or modify
% it under the terms of the GNU Affero General Public License as published
% by the Free Software Foundation, either version 3 of the License, or
% (at your option) any later version.
%
% Solution outputs
% V = u(1) = electrostatic potential
% n = u(2) = electron density
% p = u(3) = holes density
% c = u(4) = cation density (optional)
% a = u(5) = anion density (optional)
%
%% Start code
%% Deal with input arguments
if length(varargin) == 0
    % If no input parameter set then call pc directly
    par = pc;
    dficAnalytical = true;
elseif length(varargin) == 1
    % If one input argument then assume it is the Initial Conditions (IC) solution
    icsol = varargin{1, 1}.u;
    icx = varargin{1, 1}.x;
    par = varargin{1, 1}.par;
    dficAnalytical = false;
elseif length(varargin) == 2
    if max(max(max(varargin{1, 1}.u))) == 0
        par = varargin{2};
        dficAnalytical = true;
    elseif isa(varargin{2}, 'char') == 1            % Checks to see if argument is a character
        input_solstruct = varargin{1, 1};
        par = input_solstruct.par;
        icsol = input_solstruct.u;
        icx = input_solstruct.x;
        dficAnalytical = false;
    else
        input_solstruct = varargin{1, 1};
        icsol = input_solstruct.u;
        icx = input_solstruct.x;
        par = varargin{2};
        dficAnalytical = false;
    end
end

%% Unpack properties
%% Spatial mesh
xmesh = par.xx;
x_sub = par.x_sub;
x = xmesh;

%% Time mesh
t = meshgen_t(par);

%% Dependent properties: Prevents recalculation of dependent properties by pdepe defined in Methods
% Can also use AbortSet in class def
Vbi = par.Vbi;
nleft = par.nleft;
nright = par.nright;
pleft = par.pleft;
pright = par.pright;
dev = par.dev;

%% Constants
kB = par.kB;
q = par.q;
e = par.e;
epp0 = par.epp0;

%% Device parameters
device = par.dev_sub;
T = par.T;
mue = device.mue;           % Electron mobility
muh = device.muh;           % Hole mobility
Dn = mue*kB*T;              % Electron diffusion coefficient
Dp = muh*kB*T;              % Hole diffusion coefficient
mucat = device.mucat;       % Cation mobility
muani = device.muani;       % Anion mobility
Nc = device.Nc;             % Conduction band effective density of states
Nv = device.Nv;             % Valence band effective density of states
cmax = device.cmax;     % Cation density upper limit
amax = device.amax;     % Anion density upper limit
gradNc = device.gradNc;     % Conduction band effective density of states gradient
gradNv = device.gradNv;     % Valence band effective density of states gradient
gradEA = device.gradEA;     % Electron Affinity gradient
gradIP = device.gradIP;     % Ionisation Potential gradient
epp = device.epp;           % Dielectric constant
eppmax = max(par.epp);      % Maximum dielectric constant (for normalisation)
B = device.B;               % Radiative recombination rate coefficient
ni = device.ni;             % Intrinsic carrier density
taun = device.taun;         % Electron SRH time constant
taup = device.taup;         % Electron SRH time constant
taun_vsr = device.taun_vsr; % Electron SRH time constant- volumetric interfacial surface recombination scheme
taup_vsr = device.taup_vsr; % Electron SRH time constant- volumetric interfacial surface recombination scheme
nt = device.nt;             % SRH electron trap constant
pt = device.pt;             % SRH hole trap constant
NA = device.NA;             % Acceptor doping density
ND = device.ND;             % Donor doping density
Ncat = device.Ncat;         % Uniform cation density
Nani = device.Nani;         % Uniform anion density
xprime_n = device.xprime_n;         % Translated x co-ordinates for interfaces
xprime_p = device.xprime_p;         % Translated x co-ordinates for interfaces
sign_xn = device.sign_xn;           % 1 if xn increasing, -1 if decreasing wrt x
sign_xp = device.sign_xp;           % 1 if xp increasing, -1 if decreasing wrt x
alpha0_xn = device.alpha0_xn;       % alpha0_xn is alpha for F = 0 reference to xprime_n
beta0_xp = device.beta0_xp;         % beta0_xp is beta for F = 0 referenced to xprime_p
N_max_variables = par.N_max_variables;  % Maximum number of variables allowable in this version of Driftfusion
N_ionic_species = par.N_ionic_species;  % Number of ionic species in this solution
N_variables = par.N_ionic_species + 3;  % Number of variables in this solution (+3 for V, n, and p)

z_c = par.z_c;
z_a = par.z_a;
nleft = par.nleft;
nright = par.nright;
pleft = par.pleft;
pright = par.pright;
sn_l = par.sn_l;
sp_l = par.sp_l;
sn_r = par.sn_r;
sp_r = par.sp_r;
Rs = par.Rs;
Rs_initial = par.Rs_initial;

%% Switches and accelerator coefficients
mobset = par.mobset;        % Electronic carrier transport switch
mobseti = par.mobseti;      % Ionic carrier transport switch
K_cation = par.K_cation;    % Cation transport rate multiplier
K_anion = par.K_anion;      % Anion transport rate multiplier
radset = par.radset;        % Radiative recombination switch
SRHset = par.SRHset;        % SRH recombination switch
vsr_zone = device.vsr_zone;
srh_zone = device.vsr_zone;
Field_switch = device.Field_switch;

%% Generation
g1_fun = fun_gen(par.g1_fun_type);
g2_fun = fun_gen(par.g2_fun_type);
gxt1 = 0;
gxt2 = 0;
g = 0;
gx1 = par.gx1;
gx2 = par.gx2;
int1 = par.int1;
int2 = par.int2;
g1_fun_type = par.g1_fun_type;
g2_fun_type = par.g2_fun_type;
g1_fun_arg = par.g1_fun_arg;
g2_fun_arg = par.g2_fun_arg;

%% Voltage function
Vapp_fun = fun_gen(par.V_fun_type);
Vapp = 0;
Vres = 0;
J = 0;

%% Solver variables
V = 0; n = 0; p = 0; a = 0; c = 0;
dVdx = 0; dndx = 0; dpdx = 0; dadx = 0; dcdx = 0;
C_V = 0; C_n = 0; C_p = 0; C_c = 0; C_a = 0;
F_V = 0; F_n = 0; F_p = 0; F_c = 0; F_a = 0;
S_V = 0; S_n = 0; S_p = 0; S_c = 0; S_a = 0;
r_rad = 0; r_srh = 0; r_vsr = 0; r_np = 0;
alpha = 0; beta = 0;

%% Solver options
% MaxStep = limit maximum time step size during integration
options = odeset('MaxStep', par.MaxStepFactor*0.1*abs(par.tmax - par.t0), 'RelTol', par.RelTol, 'AbsTol', par.AbsTol, 'NonNegative', [1,1,1,0]);

%% Call solver
% inputs with '@' are function handles to the subfunctions
% below for the: equation, initial conditions, boundary conditions
u = pdepe(par.m,@dfpde,@dfic,@dfbc,x,t,options);

%% Ouputs
% Store final voltage reading
par.Vapp = Vapp;

% Solutions and meshes to structure
solstruct.u = u;
solstruct.x = x;
solstruct.t = t;

% Store parameters object
solstruct.par = par;

%% Volumetric surface recombination error check
if par.vsr_mode == 1 && par.vsr_check == 1
    compare_rec_flux(solstruct, par.RelTol_vsr, par.AbsTol_vsr, 0);
end

%% Subfunctions
% Set up partial differential equation (pdepe) (see MATLAB pdepe help for details of C,F,S)
% C = Time-dependence prefactor
% F = Flux terms
% S = Source terms
    function [C,F,S] = dfpde(x,t,u,dudx)
        % Get position point
        i = find(x_sub <= x);
        i = i(end);

        switch g1_fun_type
            case 'constant'
                gxt1 = int1*gx1(i);
            otherwise
                gxt1 = g1_fun(g1_fun_arg, t)*gx1(i);
        end

        switch g2_fun_type
            case 'constant'
                gxt2 = int2*gx2(i);
            otherwise
                gxt2 = g2_fun(g2_fun_arg, t)*gx2(i);
        end
        g = gxt1 + gxt2;

        %% Unpack Variables
        
        
                V = u(1);
                n = u(2);
                p = u(3);
                c = u(4);
                a = u(5);
                dVdx = dudx(1);
                dndx = dudx(2);
                dpdx = dudx(3);
                dcdx = dudx(4);
                dadx = dudx(5);












%% Equation editor
% Time-dependence prefactor term
C_V = 0; C_n = 1; C_p = 1; C_c = 1; C_a = 1;
C = [C_V; C_n; C_p; C_c; C_a];

% Flux terms
F_V = (epp(i)/eppmax)*dVdx;
F_n = mu_n(i)*n*(-dVdx + gradEA(i)) + (Dn(i)*(dndx - ((n/Nc(i))*gradNc(i))));
F_p = mu_p(i)*p*(dVdx - gradIP(i)) + (Dp(i)*(dpdx - ((p/Nv(i))*gradNv(i))));
F_c = mu_c(i)*(z_c*c*dVdx + kB*T*(dcdx + (c*(dcdx/(c_max(i) - c)))));
F_a = mu_a(i)*(z_a*a*dVdx + kB*T*(dadx + (a*(dadx/(a_max(i) - a)))));
F = [F_V; mobset*F_n; mobset*F_p; mobseti*K_c*F_c; mobseti*K_a*F_a];

% Electron and hole recombination
% Radiative
r_rad = radset*B(i)*(n*p - ni(i)^2);
% Bulk SRH
r_srh = SRHset*srh_zone(i)*((n*p - ni(i)^2)/(taun(i)*(p + pt(i)) + taup(i)*(n + nt(i))));
% Volumetric surface recombination
alpha = sign_xn(i)*q*dVdx/(kB*T) + alpha0_xn(i);
beta = sign_xp(i)*q*-dVdx/(kB*T) + beta0_xp(i);
r_vsr = SRHset*vsr_zone(i)*((n*exp(-alpha*xprime_n(i))*p*exp(-beta*xprime_p(i)) - ni(i)^2)...
    /(taun_vsr(i)*(p*exp(-beta*xprime_p(i)) + pt(i)) + taup_vsr(i)*(n*exp(-alpha*xprime_n(i)) + nt(i))));
% Total electron and hole recombination
r_np = r_rad + r_srh + r_vsr;

% Source terms
S_V = (q/(eppmax*epp0))*(-n + p - NA(i) + ND(i) + z_a*a + z_c*c - z_a*Nani(i) - z_c*Ncat(i));
S_n = g - r_np;
S_p = g - r_np;
S_c = 0;
S_a = 0;
S = [S_V; S_n; S_p; S_c; S_a];

        % Remove unused variables - faster and tidier than using conditional
        % statements
        C = C(1:N_variables);
        F = F(1:N_variables);
        S = S(1:N_variables);
    end

%% Initial conditions.
    function u0 = dfic(x)
        i = find(xmesh <= x);
        i = i(end);

        if length(par.dcell) == 1
            % Single layer
            u0_ana = [(x/xmesh(end))*Vbi;
                nleft*exp((x*(log(nright)-log(nleft)))/par.dcum0(end));
                pleft*exp((x*(log(pright)-log(pleft)))/par.dcum0(end));
                dev.Ncat(i);
                dev.Nani(i);];
        else
            % Multi-layered
            u0_ana = [(x/xmesh(end))*Vbi;
                dev.n0(i);
                dev.p0(i);
                dev.Ncat(i);
                dev.Nani(i);];
        end
        u0_ana = u0_ana(1:N_variables);

        % Organise ICs based on number of variables and SOL_IC
        if dficAnalytical
            u0 = u0_ana;
        else
            % Initial conditions taken from input solution
            u0_in = interp1(icx,squeeze(icsol(end,:,:)),x)';
            % If the number of variables has increased then add analytical
            % ICs for missing variables
            if N_variables > length(u0_in)
                % Add initial conditions for new variables from U_ANA
                u0(1:length(u0_in), 1) = u0_in;
                u0(length(u0_in)+1:N_variables, 1) = u0_ana(length(u0_in)+1:N_variables);
            else
                u0 = u0_in;
            end
        end
    end

%% Boundary conditions
% Refer to PDEPE help for the precise meaning of P and Q
% l and r refer to left and right boundaries.
    function [Pl,Ql,Pr,Qr] = dfbc(xl,ul,xr,ur,t)

        switch N_ionic_species
            case 0
                V_l = ul(1);
                V_r = ur(1);
                n_l = ul(2);
                n_r = ur(2);
                p_l = ul(3);
                p_r = ur(3);
                c_l = 0;
                c_r = 0;
                a_l = 0;
                a_r = 0;
            case 1
                V_l = ul(1);
                V_r = ur(1);
                n_l = ul(2);
                n_r = ur(2);
                p_l = ul(3);
                p_r = ur(3);
                c_l = ul(4);
                c_r = ur(4);
                a_l = 0;
                a_r = 0;
            case 2
                V_l = ul(1);
                V_r = ur(1);
                n_l = ul(2);
                n_r = ur(2);
                p_l = ul(3);
                p_r = ur(3);
                c_l = ul(4);
                c_r = ur(4);
                a_l = ul(5);
                a_r = ur(5);
        end

        switch par.V_fun_type
            case 'constant'
                Vapp = par.V_fun_arg(1);
            otherwise
                Vapp = Vapp_fun(par.V_fun_arg, t);
        end

                % Flux boundary conditions for both carrier types.
                % Calculate series resistance voltage Vres
                if Rs == 0
                    Vres = 0;
                else
                    J = e*sp_r*(ur(3) - pright) - e*sn_r*(ur(2) - nright);
                    if Rs_initial
                        Vres = -J*Rs*t/par.tmax;    % Initial linear sweep
                    else
                        Vres = -J*Rs;
                    end
                end

Pl = [-V_l;
  mobset*(-sn_l*(n_l - n0_l));
  mobset*(-sp_l*(p_l - p0_l));
  0;
  0;];

Ql = [0; 1; 1; 1; 1;];

Pr = [-V_r+Vbi-Vapp-Vres;
  mobset*(sn_r*(n_r - n0_r));
  mobset*(sp_r*(p_r - p0_r));
  0;
  0;];

Qr = [0; 1; 1; 1; 1;];


        % Remove unused entries
        Pl = Pl(1:N_variables);
        Pr = Pr(1:N_variables);
        Ql = Ql(1:N_variables);
        Qr = Qr(1:N_variables);
    end
end


==> Lst2_dfbc.tex <==
function solstruct = df(varargin)
% Core DRIFTFUSION function- organises properties and inputs for pdepe
% A routine to test solving the diffusion and drift equations using the
% matlab pepde solver.
%
%% LICENSE
% Copyright (C) 2020  Philip Calado, Ilario Gelmetti, and Piers R. F. Barnes
% Imperial College London
% This program is free software: you can redistribute it and/or modify
% it under the terms of the GNU Affero General Public License as published
% by the Free Software Foundation, either version 3 of the License, or
% (at your option) any later version.
%
% Solution outputs
% V = u(1) = electrostatic potential
% n = u(2) = electron density
% p = u(3) = holes density
% c = u(4) = cation density (optional)
% a = u(5) = anion density (optional)
%
%% Start code
%% Deal with input arguments
if length(varargin) == 0
    % If no input parameter set then call pc directly
    par = pc;
    dficAnalytical = true;
elseif length(varargin) == 1
    % If one input argument then assume it is the Initial Conditions (IC) solution
    icsol = varargin{1, 1}.u;
    icx = varargin{1, 1}.x;
    par = varargin{1, 1}.par;
    dficAnalytical = false;
elseif length(varargin) == 2
    if max(max(max(varargin{1, 1}.u))) == 0
        par = varargin{2};
        dficAnalytical = true;
    elseif isa(varargin{2}, 'char') == 1            % Checks to see if argument is a character
        input_solstruct = varargin{1, 1};
        par = input_solstruct.par;
        icsol = input_solstruct.u;
        icx = input_solstruct.x;
        dficAnalytical = false;
    else
        input_solstruct = varargin{1, 1};
        icsol = input_solstruct.u;
        icx = input_solstruct.x;
        par = varargin{2};
        dficAnalytical = false;
    end
end

%% Unpack properties
%% Spatial mesh
xmesh = par.xx;
x_sub = par.x_sub;
x = xmesh;

%% Time mesh
t = meshgen_t(par);

%% Dependent properties: Prevents recalculation of dependent properties by pdepe defined in Methods
% Can also use AbortSet in class def
Vbi = par.Vbi;
nleft = par.nleft;
nright = par.nright;
pleft = par.pleft;
pright = par.pright;
dev = par.dev;

%% Constants
kB = par.kB;
q = par.q;
e = par.e;
epp0 = par.epp0;

%% Device parameters
device = par.dev_sub;
T = par.T;
mue = device.mue;           % Electron mobility
muh = device.muh;           % Hole mobility
Dn = mue*kB*T;              % Electron diffusion coefficient
Dp = muh*kB*T;              % Hole diffusion coefficient
mucat = device.mucat;       % Cation mobility
muani = device.muani;       % Anion mobility
Nc = device.Nc;             % Conduction band effective density of states
Nv = device.Nv;             % Valence band effective density of states
cmax = device.cmax;     % Cation density upper limit
amax = device.amax;     % Anion density upper limit
gradNc = device.gradNc;     % Conduction band effective density of states gradient
gradNv = device.gradNv;     % Valence band effective density of states gradient
gradEA = device.gradEA;     % Electron Affinity gradient
gradIP = device.gradIP;     % Ionisation Potential gradient
epp = device.epp;           % Dielectric constant
eppmax = max(par.epp);      % Maximum dielectric constant (for normalisation)
B = device.B;               % Radiative recombination rate coefficient
ni = device.ni;             % Intrinsic carrier density
taun = device.taun;         % Electron SRH time constant
taup = device.taup;         % Electron SRH time constant
taun_vsr = device.taun_vsr; % Electron SRH time constant- volumetric interfacial surface recombination scheme
taup_vsr = device.taup_vsr; % Electron SRH time constant- volumetric interfacial surface recombination scheme
nt = device.nt;             % SRH electron trap constant
pt = device.pt;             % SRH hole trap constant
NA = device.NA;             % Acceptor doping density
ND = device.ND;             % Donor doping density
Ncat = device.Ncat;         % Uniform cation density
Nani = device.Nani;         % Uniform anion density
xprime_n = device.xprime_n;         % Translated x co-ordinates for interfaces
xprime_p = device.xprime_p;         % Translated x co-ordinates for interfaces
sign_xn = device.sign_xn;           % 1 if xn increasing, -1 if decreasing wrt x
sign_xp = device.sign_xp;           % 1 if xp increasing, -1 if decreasing wrt x
alpha0_xn = device.alpha0_xn;       % alpha0_xn is alpha for F = 0 reference to xprime_n
beta0_xp = device.beta0_xp;         % beta0_xp is beta for F = 0 referenced to xprime_p
N_max_variables = par.N_max_variables;  % Maximum number of variables allowable in this version of Driftfusion
N_ionic_species = par.N_ionic_species;  % Number of ionic species in this solution
N_variables = par.N_ionic_species + 3;  % Number of variables in this solution (+3 for V, n, and p)

z_c = par.z_c;
z_a = par.z_a;
nleft = par.nleft;
nright = par.nright;
pleft = par.pleft;
pright = par.pright;
sn_l = par.sn_l;
sp_l = par.sp_l;
sn_r = par.sn_r;
sp_r = par.sp_r;
Rs = par.Rs;
Rs_initial = par.Rs_initial;

%% Switches and accelerator coefficients
mobset = par.mobset;        % Electronic carrier transport switch
mobseti = par.mobseti;      % Ionic carrier transport switch
K_cation = par.K_cation;    % Cation transport rate multiplier
K_anion = par.K_anion;      % Anion transport rate multiplier
radset = par.radset;        % Radiative recombination switch
SRHset = par.SRHset;        % SRH recombination switch
vsr_zone = device.vsr_zone;
srh_zone = device.vsr_zone;
Field_switch = device.Field_switch;

%% Generation
g1_fun = fun_gen(par.g1_fun_type);
g2_fun = fun_gen(par.g2_fun_type);
gxt1 = 0;
gxt2 = 0;
g = 0;
gx1 = par.gx1;
gx2 = par.gx2;
int1 = par.int1;
int2 = par.int2;
g1_fun_type = par.g1_fun_type;
g2_fun_type = par.g2_fun_type;
g1_fun_arg = par.g1_fun_arg;
g2_fun_arg = par.g2_fun_arg;

%% Voltage function
Vapp_fun = fun_gen(par.V_fun_type);
Vapp = 0;
Vres = 0;
J = 0;

%% Solver variables
V = 0; n = 0; p = 0; a = 0; c = 0;
dVdx = 0; dndx = 0; dpdx = 0; dadx = 0; dcdx = 0;
C_V = 0; C_n = 0; C_p = 0; C_c = 0; C_a = 0;
F_V = 0; F_n = 0; F_p = 0; F_c = 0; F_a = 0;
S_V = 0; S_n = 0; S_p = 0; S_c = 0; S_a = 0;
r_rad = 0; r_srh = 0; r_vsr = 0; r_np = 0;
alpha = 0; beta = 0;

%% Solver options
% MaxStep = limit maximum time step size during integration
options = odeset('MaxStep', par.MaxStepFactor*0.1*abs(par.tmax - par.t0), 'RelTol', par.RelTol, 'AbsTol', par.AbsTol, 'NonNegative', [1,1,1,0]);

%% Call solver
% inputs with '@' are function handles to the subfunctions
% below for the: equation, initial conditions, boundary conditions
u = pdepe(par.m,@dfpde,@dfic,@dfbc,x,t,options);

%% Ouputs
% Store final voltage reading
par.Vapp = Vapp;

% Solutions and meshes to structure
solstruct.u = u;
solstruct.x = x;
solstruct.t = t;

% Store parameters object
solstruct.par = par;

%% Volumetric surface recombination error check
if par.vsr_mode == 1 && par.vsr_check == 1
    compare_rec_flux(solstruct, par.RelTol_vsr, par.AbsTol_vsr, 0);
end

%% Subfunctions
% Set up partial differential equation (pdepe) (see MATLAB pdepe help for details of C,F,S)
% C = Time-dependence prefactor
% F = Flux terms
% S = Source terms
    function [C,F,S] = dfpde(x,t,u,dudx)
        % Get position point
        i = find(x_sub <= x);
        i = i(end);

        switch g1_fun_type
            case 'constant'
                gxt1 = int1*gx1(i);
            otherwise
                gxt1 = g1_fun(g1_fun_arg, t)*gx1(i);
        end

        switch g2_fun_type
            case 'constant'
                gxt2 = int2*gx2(i);
            otherwise
                gxt2 = g2_fun(g2_fun_arg, t)*gx2(i);
        end
        g = gxt1 + gxt2;

        %% Unpack Variables
        switch N_ionic_species
            case 0
                V = u(1);
                n = u(2);
                p = u(3);
                c = 0;
                a = 0;
                dVdx = dudx(1);
                dndx = dudx(2);
                dpdx = dudx(3);
                dcdx = 0;
                dadx = 0;
            case 1
                V = u(1);
                n = u(2);
                p = u(3);
                c = u(4);
                a = Nani(i);
                dVdx = dudx(1);
                dndx = dudx(2);
                dpdx = dudx(3);
                dcdx = dudx(4);
                dadx = 0;
            case 2
                V = u(1);
                n = u(2);
                p = u(3);
                c = u(4);
                a = u(5);
                dVdx = dudx(1);
                dndx = dudx(2);
                dpdx = dudx(3);
                dcdx = dudx(4);
                dadx = dudx(5);
        end

        % Volumetric surface recombination gradients
        alpha = sign_xn(i)*q*dVdx/(kB*T) + alpha0_xn(i);
        beta = sign_xp(i)*q*-dVdx/(kB*T) + beta0_xp(i);

        %% Equation editor
        % Time-dependence prefactor term
        C_V = 0;
        C_n = 1;
        C_p = 1;
        C_c = 1;
        C_a = 1;
        C = [C_V; C_n; C_p; C_c; C_a];

        % Flux terms
        F_V = (epp(i)/eppmax)*dVdx;
        F_n = mue(i)*n*(-dVdx + gradEA(i)) + (Dn(i)*(dndx - ((n/Nc(i))*gradNc(i))));
        F_p = muh(i)*p*(dVdx - gradIP(i)) + (Dp(i)*(dpdx - ((p/Nv(i))*gradNv(i))));
        F_c = mucat(i)*(z_c*c*dVdx + kB*T*(dcdx + (c*(dcdx/(cmax(i)-c)))));
        F_a = muani(i)*(z_a*a*dVdx + kB*T*(dadx+(a*(dadx/(amax(i)-a)))));
        F = [F_V; mobset*F_n; mobset*F_p; K_cation*mobseti*F_c; K_anion*mobseti*F_a];

        % Electron and holes recombination
        % Radiative
        r_rad = radset*B(i)*((n*p)-(ni(i)^2));
        % Bulk SRH
        r_srh = SRHset*srh_zone(i)*(((n*p)-ni(i)^2)/(taun(i)*(p+pt(i)) + taup(i)*(n+nt(i))));
        % Volumetric surface recombination
        r_vsr = SRHset*vsr_zone(i)*((n*exp(-alpha*xprime_n(i))*p*exp(-beta*xprime_p(i)) - ni(i)^2)...
            /(taun_vsr(i)*(p*exp(-beta*xprime_p(i))+pt(i)) + taup_vsr(i)*(n*exp(-alpha*xprime_n(i))+nt(i))));
        % Total electron and hole recombination
        r_np = r_rad + r_srh + r_vsr;

        % Source terms
        S_V = Field_switch(i)*(q/(eppmax*epp0))*(-n + p - NA(i) + ND(i) + z_a*a + z_c*c);
        S_n = g - r_np;
        S_p = g - r_np;
        S_c = 0;
        S_a = 0;
        S = [S_V; S_n; S_p; S_c; S_a];

        % Remove unused variables - faster and tidier than using conditional
        % statements
        C = C(1:N_variables);
        F = F(1:N_variables);
        S = S(1:N_variables);
    end

%% Initial conditions.
    function u0 = dfic(x)
        i = find(xmesh <= x);
        i = i(end);

        if length(par.dcell) == 1
            % Single layer
            u0_ana = [(x/xmesh(end))*Vbi;
                nleft*exp((x*(log(nright)-log(nleft)))/par.dcum0(end));
                pleft*exp((x*(log(pright)-log(pleft)))/par.dcum0(end));
                dev.Ncat(i);
                dev.Nani(i);];
        else
            % Multi-layered
            u0_ana = [(x/xmesh(end))*Vbi;
                dev.n0(i);
                dev.p0(i);
                dev.Ncat(i);
                dev.Nani(i);];
        end
        u0_ana = u0_ana(1:N_variables);

        % Organise ICs based on number of variables and SOL_IC
        if dficAnalytical
            u0 = u0_ana;
        else
            % Initial conditions taken from input solution
            u0_in = interp1(icx,squeeze(icsol(end,:,:)),x)';
            % If the number of variables has increased then add analytical
            % ICs for missing variables
            if N_variables > length(u0_in)
                % Add initial conditions for new variables from U_ANA
                u0(1:length(u0_in), 1) = u0_in;
                u0(length(u0_in)+1:N_variables, 1) = u0_ana(length(u0_in)+1:N_variables);
            else
                u0 = u0_in;
            end
        end
    end

%% Boundary conditions
% Refer to PDEPE help for the precise meaning of P and Q
% l and r refer to left and right boundaries.
    function [Pl,Ql,Pr,Qr] = dfbc(xl,ul,xr,ur,t)

        switch N_ionic_species
            case 0
                V_l = ul(1);
                V_r = ur(1);
                n_l = ul(2);
                n_r = ur(2);
                p_l = ul(3);
                p_r = ur(3);
                c_l = 0;
                c_r = 0;
                a_l = 0;
                a_r = 0;
            case 1
                V_l = ul(1);
                V_r = ur(1);
                n_l = ul(2);
                n_r = ur(2);
                p_l = ul(3);
                p_r = ur(3);
                c_l = ul(4);
                c_r = ur(4);
                a_l = 0;
                a_r = 0;
            case 2
                V_l = ul(1);
                V_r = ur(1);
                n_l = ul(2);
                n_r = ur(2);
                p_l = ul(3);
                p_r = ur(3);
                c_l = ul(4);
                c_r = ur(4);
                a_l = ul(5);
                a_r = ur(5);
        end

        switch par.V_fun_type
            case 'constant'
                Vapp = par.V_fun_arg(1);
            otherwise
                Vapp = Vapp_fun(par.V_fun_arg, t);
        end

                % Flux boundary conditions for both carrier types.
                % Calculate series resistance voltage Vres
                if Rs == 0
                    Vres = 0;
                else
                    J = e*sp_r*(ur(3) - pright) - e*sn_r*(ur(2) - nright);
                    if Rs_initial
                        Vres = -J*Rs*t/par.tmax;    % Initial linear sweep
                    else
                        Vres = -J*Rs;
                    end
                end

Pl = [-V_l;
  mobset*(-sn_l*(n_l - n0_l));
  mobset*(-sp_l*(p_l - p0_l));
  0;
  0;];

Ql = [0; 1; 1; 1; 1;];

Pr = [-V_r+Vbi-Vapp-Vres;
  mobset*(sn_r*(n_r - n0_r));
  mobset*(sp_r*(p_r - p0_r));
  0;
  0;];

Qr = [0; 1; 1; 1; 1;];


        % Remove unused entries
        Pl = Pl(1:N_variables);
        Pr = Pr(1:N_variables);
        Ql = Ql(1:N_variables);
        Qr = Qr(1:N_variables);
    end
end


==> Lst4_doCV.tex <==
function sol_CV = doCV(sol_ini, light_intensity, V0, Vmax, Vmin, scan_rate, cycles, tpoints)
% Performs a cyclic voltammogram (CV) simulation
% Input arguments:
% SOL_INI = solution containing initial conditions
% LIGHT_INTENSITY = Light intensity for bias light (Suns)
% V0 = Starting voltage (V)
% VMAX = Maximum voltage point (V)
% VMIN = Minimum voltage point (V)
% SCAN_RATE = Scan rate (Vs-1)
% CYCLES = No. of scan cycles
% TPOINTS = No. of points in output time array
% P. Calado, 2020, Imperial College London
disp('Starting DOCV')

par = sol_ini.par;

%% Set light intensity
if light_intensity > 0
    sol = lightonRs(sol_ini, light_intensity, -1, 0, 0, 10);
else
    sol = sol_ini;
end

%% Switch to V0 if different from initial conditions
% Trying to do this within the triangular wave function resulted in
% convergence issues so safer to do this here.
if V0 ~= par.Vapp
    sol = genVappStructs(sol, V0, 0);
end

%% Calculate tmax from scan rate and absolute change in voltage, deltaV
deltaV = abs(Vmax-Vmin)+abs(Vmin-Vmax)+abs(V0-Vmin);
tmax = deltaV/scan_rate;

disp('Performing cyclic voltamagram')
sol_CV = VappFunction(sol, 'tri', [V0, Vmax, Vmin, cycles, tmax/cycles], tmax, tpoints, 0);
disp('Complete')

disp('DOCV complete')
end

==> LstS1_pc.tex <==
classdef pc
    % Authors: Philip Calado, Piers Barnes, Ilario Gelmetti, Ben Hillman, 2018 Imperial College London
    % PC (Parameters Class) defines all the required properties for your
    % device. PC.BUILDDEV builds a structure PO.DEV (where PO is a Parameters Object)
    % that defines the properties of the device at every spatial mesh point, including
    % interfaces. Whenever PROPERTIES are overwritten in a protocol, the device should
    % be rebuilt manually using PC.BUILDDEV. The spatial mesh is a linear piece-wise mesh
    % and is built by the MESHGEN_X function. Details of how to define the mesh
    % are given below in the SPATIAL MESH SUBSECTION.

    properties (Constant)
        %% Physical constants
        kB = 8.617330350e-5;     % Boltzmann constant [eV K^-1]
        epp0 = 552434;           % Epsilon_0 [e^2 eV^-1 cm^-1] - Checked (02-11-15)
        q = 1;                   % Charge of the species in units of e.
        e = 1.60217662e-19;         % Elementary charge in Coulombs.
    end

    properties
        % Temperature [K]
        T = 300;

        %% Spatial mesh
        % Device Dimensions [cm]
        % The spatial mesh is a linear piece-wise mesh and is built by the
        % MESHGEN_X function using 2 arrays DCELL and PCELL,
        % which define the thickness and number of points of each layer
        % respectively.
        dcell = 400e-7;         % Layer and subsection thickness array
        layer_points = 400;            % Points array

        %% Layer description
        % Define the layer type for each of the layers in the device. The
        % options are:
        % LAYER = standard layer
        % ACTIVE = standard layer but the properties of this layer are
        % flagged such that they can easily be accessed
        % JUNCTION = a region with graded properties between two materials
        % (either LAYER or ACTIVE type)
        % with different properties
        layer_type = {'active'}
        % STACK is used for reading the optical properties library.
        % The names here do not influence the electrical properties of the
        % device. See INDEX OF REFRACTION LIBRARY for choices- names must be entered
        % exactly as given in the column headings with the '_n', '_k' omitted
        stack = {'MAPICl'}

        % Define spatial cordinate system- typically this will be kept at
        % 0 for most applications
        % m=0 cartesian
        % m=1 cylindrical polar coordinates
        % m=2 spherical polar coordinates
        m = 0;

        %% Spatial mesh
        % xmesh_type specification - see MESHGEN_X.
        xmesh_type = 5;
        xmesh_coeff = [0.7];        % Coefficient array for defining point spacing
        
        %% Time mesh
        % The time mesh is dynamically generated by ODE15s- the mesh
        % defined by MESHGEN_T only defines the values of the points that
        % are read out and so does not influence convergence. Defining an
        % unecessarily high number of points however can be expensive owing
        % to interpolation of the solution.
        tmesh_type = 2;             % Mesh type- for use with meshgen_t
        t0 = 1e-16;                 % Initial log mesh time value
        tmax = 1e-12;               % Max time value
        tpoints = 100;              % Number of time points

        %% GENERAL CONTROL PARAMETERS
        OC = 0;                 % Closed circuit = 0, Open Circuit = 1
        Vapp = 0;               % Applied bias
        BC = 3;                 % Boundary Conditions. Must be set to one for first solution
        figson = 1;             % Toggle figures on/off
        meshx_figon = 0;        % Toggles x-mesh figures on/off
        mesht_figon = 0;        % Toggles t-mesh figures on/off
        side = 1;               % illumination side 1 = left, 2 = right
        calcJ = 0;              % Calculates Currents- slows down solving calcJ = 1, calculates DD currents at every position
        mobset = 1;             % Switch on/off electron hole mobility- MUST BE SET TO ZERO FOR INITIAL SOLUTION
        mobseti = 1;
        SRHset = 1;
        radset = 1;
        JV = 0;                 % Toggle run JV scan on/off
        prob_distro_function = 'Boltz';        % 'Fermi' = Fermi-Dirac, % 'Boltz' = Boltzmann statistics
        Fermi_limit = 0.2;      % Max allowable limit for Fermi levels beyond the bands [eV]
        Fermi_Dn_points = 400;  % No. of points in the Fermi-Dirac look-up table
        intgradfun = 'linear'      % Interface gradient function 'linear' = linear, 'erf' = 'error function'

        %% Generation
        % OM = Optical Model
        % 0 = Uniform Generation
        % 1 = Beer Lambert
        OM = 1;
        Int = 0;                % Bias Light intensity (multiples of g0 or 1 sun for Beer-Lambert)
        int1 = 0;
        int2 = 0;
        g0 = [2.6409e+21];      % Uniform generation rate [cm-3s-1]
        light_source1 = 'AM15';
        light_source2 = 'laser';
        laser_lambda1 = 0;
        laser_lambda2 = 638;
        g1_fun_type = 'constant'
        g2_fun_type = 'constant'
        g1_fun_arg = 0;
        g2_fun_arg = 0;
        % default: Approximate Uniform generation rate @ 1 Sun for 510 nm active layer thickness

        %% Pulse settings
        pulsepow = 10;          % Pulse power [mW cm-2] OM2 (Beer-Lambert and Transfer Matrix only)

        %%%%%%%%%%% LAYER MATERIAL PROPERTIES %%%%%%%%%%%%%%%%%%%%
        % Numerical values should be given as a row vector with the number of
        % entries equal to the number of layers specified in STACK

        %% Energy levels [eV]
        EA = [0];           % Electron affinity
        IP = [-1];           % Ionisation potential

        %% Equilibrium Fermi energies [eV]
        % These define the doping density in each layer- see NA and ND calculations in methods
        E0 = [-0.5];

        %% SRH trap energies [eV]
        % These must exist within the energy gap of the appropriate layers
        % and define the variables PT and NT in the expression:
        % U = (np-ni^2)/(taun(p+pt) +taup(n+nt))
        Et =[-0.5];

        %% Electrode Fermi energies [eV]
        % Fermi energies of the metal electrode. These define the built-in voltage, Vbi
        % and the boundary carrier concentrations nleft, pleft, nright, and
        % pright
        Phi_left = -0.6;
        Phi_right = -0.4;

        %% Effective Density Of States (eDOS) [cm-3]
        Nc = [1e19];
        Nv = [1e19];
        % PEDOT eDOS: https://aip.scitation.org/doi/10.1063/1.4824104
        % MAPI eDOS: F. Brivio, K. T. Butler, A. Walsh and M. van Schilfgaarde, Phys. Rev. B, 2014, 89, 155204.
        % PCBM eDOS:

%% Mobile ions
% Mobile ion defect density [cm-3]
N_ionic_species = 1;
K_anion = 1;         % Coefficients to easily accelerate ions
K_cation = 1;        % Coefficients to easily accelerate ions
Nani = [1e19];
Ncat = [1e19];
% Approximate density of iodide sites [cm-3]
% Limits the density of iodide vancancies
a_max = [1.21e22];
c_max = [1.21e22]; 
% Ionic generation and recombination rates
k_iongen = [0];
k_ionrec = [0];
        
%% Mobilities   [cm2V-1s-1]
mu_n = [1];         % electron mobility
mu_p = [1];         % hole mobility

mu_a = [1e-10];          % ion mobility
mu_c = [1e-14];
        

        
        % PTPD h+ mobility: https://pubs.rsc.org/en/content/articlehtml/2014/ra/c4ra05564k
        % PEDOT mue = 0.01 cm2V-1s-1 https://aip.scitation.org/doi/10.1063/1.4824104
        % TiO2 mue = 0.09 cm2V-1s-1 Bak2008
        % Spiro muh = 0.02 cm2V-1s-1 Hawash2018

        %% Relative dielectric constants
        epp = [10];

        %% Recombination
        % Radiative recombination, U = k(np - ni^2)
        % [cm3 s-1] Radiative Recombination coefficient
        krad = [3.6e-12];

        %% SRH time constants for each layer [s]
        taun = [1e6];           % [s] SRH time constant for electrons
        taup = [1e6];           % [s] SRH time constant for holes

        %% Surface recombination and extraction coefficients [cm s-1]
        % Descriptions given in the comments considering that holes are
        % extracted at left boundary, electrons at right boundary
        sn_l = 1e7;     % electron surface recombination velocity left boundary
        sn_r = 1e7;     % electron extraction velocity right boundary
        sp_l = 1e7;     % hole extraction left boundary
        sp_r = 1e7;     % hole surface recombination velocity right boundary

        %% Series resistance
        Rs = 0;
        Rs_initial = 0;         % Switch to allow linear ramp of Rs on first application

        %% Dynamically created variables
        genspace = [];
        x = [];
        xx = [];
        x_ihalf = [];
        dev = [];
        dev_ihalf = [];
        t = [];
        xpoints = [];
        gx1 = [];       % Light source 1
        gx2 = [];       % Light source 2

        %% Voltage function parameters
        V_fun_type = 'constant';
        V_fun_arg = 0;
        
        % Define the default relative tolerance for the pdepe solver
        % 1e-3 is the default, can be decreased if more precision is needed
        % Solver options
        MaxStepFactor = 1;      % Multiplier for easy access to maximum time step
        RelTol = 1e-3;
        AbsTol = 1e-6;
        
        %% Impedance parameters
        J_E_func = [];
        J_E_func_tilted = [];
        E2_func = [];
    end

    %%  Properties whose values depend on other properties (see 'get' methods).
    properties (Dependent)
        active_layer
        d
        parr
        d_active
        dcum
        dcum0           % includes first entry as zero
        d_midactive
        dEAdx
        dIPdx
        dNcdx
        dNvdx
        Dn
        Eg
        Eif
        NA
        ND
        Vbi
        n0
        nleft
        nright
        ni
        nt_bulk         % Density of CB electrons when Fermi level at trap state energy
        nt_inter
        p0
        pcum
        pcum0           % Includes first entry as zero
        pleft
        pright
        pt_bulk         % Density of VB holes when Fermi level at trap state energy
        pt_inter
        wn
        wp
        wscr            % Space charge region width
        x0              % Initial spatial mesh value

    end

    methods
        function par = pc(varargin)
            % Parameters constructor function- runs numerous checks that
            % the input properties are consistent with the model
            if length(varargin) == 1
                % Use argument as filepath and overwrite properties using
                % PC.IMPORTPROPERTIES
                filepath = varargin;
                par = import_properties(par, filepath);
            elseif length(varargin) > 1
                filepath = varargin{1, 1};
                warning('pc should have 0 or 1 input arguments- only the first argument will be used for the filepath')
            end

            % Warn if tmesh_type is not correct
            if ~ any([1 2 3 4] == par.tmesh_type)
                warning('PARAMS.tmesh_type should be an integer from 1 to 3 inclusive. MESHGEN_T cannot generate a mesh if this is not the case.')
            end

            % Warn if xmesh_type is not correct
            if ~ any(1:1:5 == par.xmesh_type)
                warning('PARAMS.xmesh_type should be an integer from 1 to 5 inclusive. MESHGEN_X cannot generate a mesh if this is not the case.')
            end

            % Warn if doping density exceeds eDOS
            for i = 1:length(par.ND)
                if par.ND(i) > par.Nc(i) || par.NA(i) > par.Nc(i)
                    msg = 'Doping density must be less than eDOS. For consistent values ensure electrode workfunctions are within the band gap and check expressions for doping density in Dependent variables.';
                    error(msg);
                end
            end

            % Warn if trap energies are outside of band gap energies
            for i = 1:length(par.Et)
                if par.Et(i) >= par.EA(i) || par.Et(i) <= par.IP(i)
                    msg = 'Trap energies must exist within layer band gap.';
                    error(msg);
                end
            end

            % Warn if DOSani is set to zero in any layers - leads to
            % infinite diffusion rate
            for i = 1:length(par.DOSani)
                if par.DOSani(i) <= 0
                    msg = 'ion DOS (DOSani) cannot have zero or negative entries- choose a low value rather than zero e.g. 1';
                    error(msg);
                end
            end

            % Warn if electrode workfunctions are outside of boundary layer
            % bandgap
            if par.Phi_left < par.IP(1) || par.Phi_left > par.EA(1)
                msg = 'Left-hand workfunction (Phi_left) out of range: value must exist within left-hand layer band gap';
                error(msg)
            end

            if par.Phi_right < par.IP(end) || par.Phi_right > par.EA(end)
                msg = 'Right-hand workfunction (Phi_right) out of range: value must exist within right-hand layer band gap';
                error(msg)
            end

            % Warn if property array do not have the correct number of
            % layers. The layer thickness array is used to define the
            % number of layers
            if length(par.parr) ~= length(par.d)
                msg = 'Points array (parr) does not have the correct number of elements. Property arrays must have the same number of elements as the thickness array (d), except SRH properties for interfaces which should have length(d)-1 elements.';
                error(msg);
            elseif length(par.EA) ~= length(par.d)
                msg = 'Electron Affinity array (EA) does not have the correct number of elements. Property arrays must have the same number of elements as the thickness array (d), except SRH properties for interfaces which should have length(d)-1 elements.';
                error(msg);
            elseif length(par.IP) ~= length(par.d)
                msg = 'Ionisation Potential array (IP) does not have the correct number of elements. Property arrays must have the same number of elements as the thickness array (d), except SRH properties for interfaces which should have length(d)-1 elements.';
                error(msg);
            elseif length(par.mue) ~= length(par.d)
                msg = 'Electron mobility array (mue) does not have the correct number of elements. Property arrays must have the same number of elements as the thickness array (d), except SRH properties for interfaces which should have length(d)-1 elements.';
                error(msg);
            elseif length(par.muh) ~= length(par.d)
                msg = 'Hole mobility array (mue) does not have the correct number of elements. Property arrays must have the same number of elements as the thickness array (d), except SRH properties for interfaces which should have length(d)-1 elements.';
                error(msg);
            elseif length(par.muani) ~= length(par.d)
                msg = 'Ion mobility array (muh) does not have the correct number of elements. Property arrays must have the same number of elements as the thickness array (d), except SRH properties for interfaces which should have length(d)-1 elements.';
                error(msg);
            elseif length(par.NA) ~= length(par.d)
                msg = 'Acceptor density array (NA) does not have the correct number of elements. Property arrays must have the same number of elements as the thickness array (d), except SRH properties for interfaces which should have length(d)-1 elements.';
                error(msg);
            elseif length(par.ND) ~= length(par.d)
                msg = 'Donor density array (ND) does not have the correct number of elements. Property arrays must have the same number of elements as the thickness array (d), except SRH properties for interfaces which should have length(d)-1 elements.';
                error(msg);
            elseif length(par.Nc) ~= length(par.d)
                msg = 'Effective density of states array (Nc) does not have the correct number of elements. Property arrays must have the same number of elements as the thickness array (d), except SRH properties for interfaces which should have length(d)-1 elements.';
                error(msg);
            elseif length(par.Nv) ~= length(par.d)
                msg = 'Effective density of states array (Nv) does not have the correct number of elements. Property arrays must have the same number of elements as the thickness array (d), except SRH properties for interfaces which should have length(d)-1 elements.';
                error(msg);
            elseif length(par.Nani) ~= length(par.d)
                msg = 'Background ion density (Nani) does not have the correct number of elements. Property arrays must have the same number of elements as the thickness array (d), except SRH properties for interfaces which should have length(d)-1 elements.';
                error(msg);
            elseif length(par.DOSani) ~= length(par.d)
                msg = 'Ion density of states array (DOSani) does not have the correct number of elements. Property arrays must have the same number of elements as the thickness array (d), except SRH properties for interfaces which should have length(d)-1 elements.';
                error(msg);
            elseif length(par.epp) ~= length(par.d)
                msg = 'Relative dielectric constant array (epp) does not have the correct number of elements. Property arrays must have the same number of elements as the thickness array (d), except SRH properties for interfaces which should have length(d)-1 elements.';
                error(msg);
            elseif length(par.krad) ~= length(par.d)
                msg = 'Radiative recombination coefficient array (krad) does not have the correct number of elements. Property arrays must have the same number of elements as the thickness array (d), except SRH properties for interfaces which should have length(d)-1 elements.';
                error(msg);
            elseif length(par.E0) ~= length(par.d)
                msg = 'Equilibrium Fermi level array (E0) does not have the correct number of elements. Property arrays must have the same number of elements as the thickness array (d), except SRH properties for interfaces which should have length(d)-1 elements.';
                error(msg);
            elseif length(par.g0) ~= length(par.d)
                msg = 'Uniform generation array (g0) does not have the correct number of elements. Property arrays must have the same number of elements as the thickness array (d), except SRH properties for interfaces which should have length(d)-1 elements.';
                error(msg);
            elseif length(par.taun) ~= length(par.d)
                msg = 'Bulk SRH electron time constants array (taun_bulk) does not have the correct number of elements. Property arrays must have the same number of elements as the thickness array (d), except SRH properties for interfaces which should have length(d)-1 elements.';
                error(msg);
            elseif length(par.taup) ~= length(par.d)
                msg = 'Bulk SRH hole time constants array (taup_bulk) does not have the correct number of elements. Property arrays must have the same number of elements as the thickness array (d), except SRH properties for interfaces which should have length(d)-1 elements.';
                error(msg);
            elseif length(par.Et) ~= length(par.d)
                msg = 'Bulk SRH trap energy array (Et) does not have the correct number of elements. Property arrays must have the same number of elements as the thickness array (d), except SRH properties for interfaces which should have length(d)-1 elements.';
                error(msg);
            end

            %% Device and generation builder
            % Import variables and structure, xx, gx1, gx2, and dev must be
            % refreshed when to rebuild the device for example when
            % changing device thickness on the fly. These are not present
            % in the dependent variables as it is too costly to have them
            % continuously called.
            par = refresh_device(par);
        end

        function par = set.xmesh_type(par, value)
            %   SET.xmesh_type(PARAMS, VALUE) checks if VALUE is an integer
            %   from 1 to 3, and if so, changes PARAMS.xmesh_type to VALUE.
            %   Otherwise, a warning is shown. Runs automatically whenever
            %   xmesh_type is changed.
            if any(1:1:5 == value)
                par.xmesh_type = value;
            else
                error('PARAMS.xmesh_type should be an integer from 1 to 3 inclusive. MESHGEN_X cannot generate a mesh if this is not the case.')
            end
        end

        function par = set.tmesh_type(par, value)
            %   SET.tmesh_type(PARAMS, VALUE) checks if VALUE is an integer
            %   from 1 to 2, and if so, changes PARAMS.tmesh_type to VALUE.
            %   Otherwise, a warning is shown. Runs automatically whenever
            %   tmesh_type is changed.
            if any(1:1:4 == value)
                par.tmesh_type = value;
            else
                error('PARAMS.tmesh_type should be an integer from 1 to 4 inclusive. MESHGEN_T cannot generate a mesh if this is not the case.')
            end
        end

        function par = set.ND(par, value)
            for i = 1:length(par.ND)
                if value(i) >= par.Nc(i)
                    error('Doping density must be less than eDOS. For consistent values ensure electrode workfunctions are within the band gap.')
                end
            end
        end

        function par = set.NA(par, value)
            for i = 1:length(par.ND)
                if value(i) >= par.Nv(i)
                    error('Doping density must be less than eDOS. For consistent values ensure electrode workfunctions are within the band gap.')
                end
            end
        end

        %% Get active layer indexes from layer_type
        function value = get.active_layer(par)
            value = find(strncmp('active', par.layer_type,6));
            if length(value) == 0
                % If no flag is give assume active layer is middle
                value = round(length(par.layer_type)/2);
            end
        end

        %% Active layer thickness
        function value = get.d_active(par)
            value = sum(par.dcell(par.active_layer(1):par.active_layer(end)));
        end
    
        function value = get.d_midactive(par)
           value = par.dcum(par.active_layer(1)-1) + par.d_active/2;
        end
        %% Layer thicknesses [cm]
        function value = get.d(par)
            % For backwards comptibility. layer_points and parr arre the now the
            % same thing
            value = par.dcell;
        end

        %% Layer points
        function value = get.parr(par)
            % For backwards comptibility. layer_points and parr arre the now the
            % same thing
            value = par.layer_points;
        end

        %% Band gap energies    [eV]
        function value = get.Eg(par)
            value = par.EA - par.IP;
        end

        %% Built-in voltage Vbi based on difference in boundary workfunctions
        function value = get.Vbi(par)
            value = par.Phi_right - par.Phi_left;
        end

        %% Intrinsic Fermi Energies
        % Currently uses Boltzmann stats as approximation should always be
        function value = get.Eif(par)
            value = 0.5.*(par.EA+par.IP)+par.kB*par.T*log(par.Nc./par.Nv);
        end

        %% Donor densities
        function value = get.ND(par)
            value = zeros(1, length(par.stack));
            value = distro_fun.nfun(par.Nc, par.EA, par.E0, par.T, par.prob_distro_function);
        end

        %% Acceptor densities
        function value = get.NA(par)
            value = zeros(1, length(par.stack));
            value = distro_fun.pfun(par.Nv, par.IP, par.E0, par.T, par.prob_distro_function);
        end

        %% Intrinsic carrier densities (Boltzmann)
        function value = get.ni(par)
            value = par.Nc.*exp(-par.Eg./(2*par.kB*par.T));
        end

        %% Equilibrium electron densities
        function value = get.n0(par)
            value = distro_fun.nfun(par.Nc, par.EA, par.E0, par.T, par.prob_distro_function);
        end

        %% Equilibrium hole densities
        function value = get.p0(par)
            value = distro_fun.pfun(par.Nv, par.IP, par.E0, par.T, par.prob_distro_function);

        end

        %% Boundary electron and hole densities
        % Uses metal Fermi energies to calculate boundary densities
        % Electrons left boundary
        function value = get.nleft(par)
            value = distro_fun.nfun(par.Nc(1), par.EA(1), par.Phi_left, par.T, par.prob_distro_function);
        end

        % Electrons right boundary
        function value = get.nright(par)
            value = distro_fun.nfun(par.Nc(end), par.EA(end), par.Phi_right, par.T, par.prob_distro_function);
        end

        % Holes left boundary
        function value = get.pleft(par)
            value = distro_fun.pfun(par.Nv(1), par.IP(1), par.Phi_left, par.T, par.prob_distro_function);
        end

        % holes right boundary
        function value = get.pright(par)
            value = distro_fun.pfun(par.Nv(end), par.IP(end), par.Phi_right, par.T, par.prob_distro_function);
        end

        function value = get.dcum(par)
            value = cumsum(par.dcell);
        end

        function value = get.pcum(par)
            value = cumsum(par.layer_points);
        end

        function value = get.pcum0(par)
            value = [1, cumsum(par.layer_points)];
        end

        function value = get.dcum0(par)
            value = [0, cumsum(par.dcell)];
        end
    end

    methods (Static)

        function xx = xmeshini(par) % For backwards compatibility
            xx = meshgen_x(par);
        end     

    end
end


==> LstS3_import_properties.tex <==
function par = import_properties(par, filepath)
% A function to IMPORT_PROPERTIES from a text file LOCATED at FILEPATH. Each of the listed properties
% is checked to see if it is available in the .CSV file. If it is available, the existing properties
% are overwritten otherwise a warning is displayed.

T = readtable(filepath{1,1});   % Reads-in in the external .CSV file to a table T

try
    par.layer_type = T{:,'layer_type'}';
catch
    warning('No layer type (layer_type) defined in .csv . Using default in PC')
end
try
    par.stack = T{:,'stack'}';
catch
    warning('No stack (stack) defined in .csv . Using default in PC')
end
try
    par.dcell = T{:, 'thickness'}';
catch
    warning('No thickness array (thickness) defined in .csv . Using default in PC')
end
try
    par.layer_points = T{:, 'layer_points'}';
catch
    warning('No layer points array (points) defined in .csv . Using default in PC')
end
try
    par.xmesh_coeff = T{:, 'xmesh_coeff'}';
catch
    warning('No xmesh coefficient array (xmesh_coeff) defined in .csv . Using default in PC')
end
try
    par.EA = T{:, 'EA'}';
catch
    warning('No electron affinity array (EA) defined in .csv . Using default in PC')
end
try
    par.IP = T{:, 'IP'}';
catch
    warning('No ionisation potential array (IP) defined in .csv . Using default in PC')
end
try
    par.E0 = T{:, 'E0'}';
catch
    warning('No equilibrium Fermi level array (E0) defined in .csv . Using default in PC')
end
try
    par.Nc = T{:, 'Nc'}';
catch
    warning('No conduction band eDOS array (Nc) defined in .csv . Using default in PC')
end
try
    par.Nv = T{:, 'Nv'}';
catch
    warning('No valence band eDOS array (Nv) defined in .csv . Using default in PC')
end
try
    par.Nani = T{:, 'Nani'}';
catch
    warning('No equilibrium anion density array (Nani) defined in .csv . Using default in PC')
end
try
    par.Ncat = T{:, 'Ncat'}';
catch
    warning('No equilibrium cation density array (Ncat) defined in .csv . Using default in PC')
end
try
    par.DOSani = T{:, 'DOSani'}';
catch
    warning('No maximum anion density array (DOSani) defined in .csv . Using default in PC')
end
try
    par.DOScat = T{:, 'DOScat'}';
catch
    warning('No maximum cation density array (DOScat) defined in .csv . Using default in PC')
end
try
    par.mue = T{:, 'mue'}';
catch
    warning('No electron mobility (mue) defined in .csv . Using default in PC')
end
try
    par.muh = T{:, 'muh'}';
catch
    warning('No hole mobility (muh) defined in .csv . Using default in PC')
end

try
    par.muani = T{:, 'muani'}';
catch
    warning('No anion mobility (muani) defined in .csv . Using default in PC')
end
try
    par.mucat = T{:, 'mucat'}';
catch
    warning('No cation mobility (mucat) defined in .csv . Using default in PC')
end
try
    par.epp = T{:, 'epp'}';
catch
    warning('No relative dielectric constant (epp) defined in .csv . Using default in PC')
end

try
    par.g0 = T{:, 'g0'}';
catch
    warning('No uniform generation rate (g0) defined in .csv . Using default in PC')
end
try
    par.krad = T{:, 'krad'}';
catch
    warning('No radiative recombinaiton coefficient array (krad) defined in .csv . Using default in PC')
end

try
    par.taun = T{:, 'taun'}';
catch
    warning('No SRH electron lifetime array (taun) defined in .csv . Using default in PC')
end
try
    par.taup = T{:, 'taup'}';
catch
    warning('No SRH hole lifetime array (taup) defined in .csv . Using default in PC')
end
try
    par.sn_l = T{1, 'sn_l'}';
catch
    warning('No sn_l defined in .csv . Using default in PC')
end
try
    par.sp_l = T{1, 'sp_l'}';
catch
    warning('No sp_l defined in .csv . Using default in PC')
end
try
    par.sn_r = T{1, 'sn_r'}';
catch
    warning('No sn_r defined in .csv . Using default in PC')
end
try
    par.sp_r = T{1, 'sp_r'}';
catch
    warning('No sp_r defined in .csv . Using default in PC')
end

try
    par.Phi_left = T{1, 'Phi_left'};
catch
    warning('No Phi_left defined in .csv . Using default in PC')
end
try
    par.Phi_right = T{1, 'Phi_right'};
catch
    warning('No Phi_right defined in .csv . Using default in PC')
end
try
    par.Et = T{:,'Et'}';
catch
    warning('No trap energy array (Et) defined in .csv . Using default in PC')
end
try
    par.OM = T{1, 'OM'};
catch
    warning('No optical model (OM) specified in .csv Using default in PC')
end
try
    par.xmesh_type = T{1, 'xmesh_type'};
catch
    warning('No spatial mesh type (xmesh_type) defined in .csv . Using default in PC')
end
try
    par.side = T{1, 'side'};
catch
    warning('Illumination side (side) undefined in .csv . Using default in PC')
end
try
    par.N_ionic_species = T{1, 'N_ionic_species'};
catch
    warning('No of ionic species (N_ionic_species) undefined in .csv. Using default in PC')
end
try
    par.k_iongen = T{1, 'k_iongen'};
catch
    warning('k_iongen undefined in .csv. Using default in PC')
end
try
    par.k_ionrec = T{1, 'k_ionrec'};
catch
    warning('k_ionrec undefined in .csv. Using default in PC')
end

%% Additional checks for backwards compatibility- old variable names
% No warning required otherwise will constantly warn when building
% parameters object
try
    par.Nani = T{:, 'Nion'}';
end
try
    par.DOSani = T{:, 'DOSion'}';
end
try
    par.muani = T{:, 'muion'}';
end
try
    par.Et = T{:,'Et_bulk'}';
end
try
    par.taun = T{:, 'taun_SRH'}';
end
try
    par.taup = T{:, 'taup_SRH'}';
end
try
    par.g0 = T{:, 'G0'}';
end
try
    par.Phi_left = T{1, 'PhiA'};
end
try
    par.Phi_right = T{1, 'PhiC'}; 
end
try
    par.layer_points = T{:, 'points'}';
end
end

==> LstS4_df_ion_gen.tex <==
function solstruct = df(varargin)
% Core DRIFTFUSION function- organises properties and inputs for pdepe
% A routine to test solving the diffusion and drift equations using the
% matlab pepde solver.
%
%% LICENSE
% Copyright (C) 2020  Philip Calado, Ilario Gelmetti, and Piers R. F. Barnes
% Imperial College London
% This program is free software: you can redistribute it and/or modify
% it under the terms of the GNU Affero General Public License as published
% by the Free Software Foundation, either version 3 of the License, or
% (at your option) any later version.
%
% Solution outputs
% V = u(1) = electrostatic potential
% n = u(2) = electron density
% p = u(3) = holes density
% c = u(4) = cation density (optional)
% a = u(5) = anion density (optional)
%
%% Start code
%% Deal with input arguments
if length(varargin) == 0
    % If no input parameter set then call pc directly
    par = pc;
    dficAnalytical = true;
elseif length(varargin) == 1
    % If one input argument then assume it is the Initial Conditions (IC) solution
    icsol = varargin{1, 1}.u;
    icx = varargin{1, 1}.x;
    par = varargin{1, 1}.par;
    dficAnalytical = false;
elseif length(varargin) == 2
    if max(max(max(varargin{1, 1}.u))) == 0
        par = varargin{2};
        dficAnalytical = true;
    elseif isa(varargin{2}, 'char') == 1            % Checks to see if argument is a character
        input_solstruct = varargin{1, 1};
        par = input_solstruct.par;
        icsol = input_solstruct.u;
        icx = input_solstruct.x;
        dficAnalytical = false;
    else
        input_solstruct = varargin{1, 1};
        icsol = input_solstruct.u;
        icx = input_solstruct.x;
        par = varargin{2};
        dficAnalytical = false;
    end
end

%% Unpack properties
%% Spatial mesh
xmesh = par.xx;
x_sub = par.x_sub;
x = xmesh;

%% Time mesh
t = meshgen_t(par);

%% Dependent properties: Prevents recalculation of dependent properties by pdepe defined in Methods
% Can also use AbortSet in class def
Vbi = par.Vbi;
nleft = par.nleft;
nright = par.nright;
pleft = par.pleft;
pright = par.pright;
dev = par.dev;

%% Constants
kB = par.kB;
q = par.q;
e = par.e;
epp0 = par.epp0;

%% Device parameters
device = par.dev_sub;
T = par.T;
mue = device.mue;           % Electron mobility
muh = device.muh;           % Hole mobility
Dn = mue*kB*T;              % Electron diffusion coefficient
Dp = muh*kB*T;              % Hole diffusion coefficient
mucat = device.mucat;       % Cation mobility
muani = device.muani;       % Anion mobility
Nc = device.Nc;             % Conduction band effective density of states
Nv = device.Nv;             % Valence band effective density of states
cmax = device.cmax;     % Cation density upper limit
amax = device.amax;     % Anion density upper limit
gradNc = device.gradNc;     % Conduction band effective density of states gradient
gradNv = device.gradNv;     % Valence band effective density of states gradient
gradEA = device.gradEA;     % Electron Affinity gradient
gradIP = device.gradIP;     % Ionisation Potential gradient
epp = device.epp;           % Dielectric constant
eppmax = max(par.epp);      % Maximum dielectric constant (for normalisation)
B = device.B;               % Radiative recombination rate coefficient
ni = device.ni;             % Intrinsic carrier density
taun = device.taun;         % Electron SRH time constant
taup = device.taup;         % Electron SRH time constant
taun_vsr = device.taun_vsr; % Electron SRH time constant- volumetric interfacial surface recombination scheme
taup_vsr = device.taup_vsr; % Electron SRH time constant- volumetric interfacial surface recombination scheme
k_iongen = device.k_iongen; % Ion generation coefficient
k_ionrec = device.k_ionrec; % Ion recombination coefficient
nt = device.nt;             % SRH electron trap constant
pt = device.pt;             % SRH hole trap constant
NA = device.NA;             % Acceptor doping density
ND = device.ND;             % Donor doping density
Ncat = device.Ncat;         % Uniform cation density
Nani = device.Nani;         % Uniform anion density
xprime_n = device.xprime_n;         % Translated x co-ordinates for interfaces
xprime_p = device.xprime_p;         % Translated x co-ordinates for interfaces
sign_xn = device.sign_xn;           % 1 if xn increasing, -1 if decreasing wrt x
sign_xp = device.sign_xp;           % 1 if xp increasing, -1 if decreasing wrt x
alpha0_xn = device.alpha0_xn;       % alpha0_xn is alpha for F = 0 reference to xprime_n
beta0_xp = device.beta0_xp;         % beta0_xp is beta for F = 0 referenced to xprime_p
N_max_variables = par.N_max_variables;  % Maximum number of variables allowable in this version of Driftfusion
N_ionic_species = par.N_ionic_species;  % Number of ionic species in this solution
N_variables = par.N_ionic_species + 3;  % Number of variables in this solution (+3 for V, n, and p)

z_c = par.z_c;
z_a = par.z_a;
nleft = par.nleft;
nright = par.nright;
pleft = par.pleft;
pright = par.pright;
sn_l = par.sn_l;
sp_l = par.sp_l;
sn_r = par.sn_r;
sp_r = par.sp_r;
Rs = par.Rs;
Rs_initial = par.Rs_initial;

%% Switches and accelerator coefficients
mobset = par.mobset;        % Electronic carrier transport switch
mobseti = par.mobseti;      % Ionic carrier transport switch
K_cation = par.K_cation;    % Cation transport rate multiplier
K_anion = par.K_anion;      % Anion transport rate multiplier
radset = par.radset;        % Radiative recombination switch
SRHset = par.SRHset;        % SRH recombination switch
vsr_zone = device.vsr_zone;

%% Generation
g1_fun = fun_gen(par.g1_fun_type);
g2_fun = fun_gen(par.g2_fun_type);
gxt1 = 0;
gxt2 = 0;
g = 0;
gx1 = par.gx1;
gx2 = par.gx2;
int1 = par.int1;
int2 = par.int2;
g1_fun_type = par.g1_fun_type;
g2_fun_type = par.g2_fun_type;
g1_fun_arg = par.g1_fun_arg;
g2_fun_arg = par.g2_fun_arg;

%% Voltage function
Vapp_fun = fun_gen(par.V_fun_type);
Vapp = 0;
Vres = 0;
J = 0;

%% Solver variables
V = 0; n = 0; p = 0; a = 0; c = 0;
dVdx = 0; dndx = 0; dpdx = 0; dadx = 0; dcdx = 0;
C_V = 0; C_n = 0; C_p = 0; C_c = 0; C_a = 0;
F_V = 0; F_n = 0; F_p = 0; F_c = 0; F_a = 0;
S_V = 0; S_n = 0; S_p = 0; S_c = 0; S_a = 0;
r_rad = 0; r_srh = 0; r_vsr = 0; r_np = 0;
alpha = 0; beta = 0;

%% Solver options
% MaxStep = limit maximum time step size during integration
options = odeset('MaxStep', par.MaxStepFactor*0.1*abs(par.tmax - par.t0), 'RelTol', par.RelTol, 'AbsTol', par.AbsTol, 'NonNegative', [1,1,1,0]);

%% Call solver
% inputs with '@' are function handles to the subfunctions
% below for the: equation, initial conditions, boundary conditions
u = pdepe(par.m,@dfpde,@dfic,@dfbc,x,t,options);

%% Ouputs
% Store final voltage reading
par.Vapp = Vapp;

% Solutions and meshes to structure
solstruct.u = u;
solstruct.x = x;
solstruct.t = t;

% Store parameters object
solstruct.par = par;

%% Volumetric surface recombination error check
if par.vsr_mode == 1 && par.vsr_check == 1
    compare_rec_flux(solstruct, par.RelTol_vsr, par.AbsTol_vsr, 0);
end

%% Subfunctions
% Set up partial differential equation (pdepe) (see MATLAB pdepe help for details of C,F,S)
% C = Time-dependence prefactor
% F = Flux terms
% S = Source terms
    function [C,F,S] = dfpde(x,t,u,dudx)
        % Get position point
        i = find(x_sub <= x);
        i = i(end);

        switch g1_fun_type
            case 'constant'
                gxt1 = int1*gx1(i);
            otherwise
                gxt1 = g1_fun(g1_fun_arg, t)*gx1(i);
        end

        switch g2_fun_type
            case 'constant'
                gxt2 = int2*gx2(i);
            otherwise
                gxt2 = g2_fun(g2_fun_arg, t)*gx2(i);
        end
        g = gxt1 + gxt2;

        %% Unpack Variables
        
        
                V = u(1);
                n = u(2);
                p = u(3);
                c = u(4);
                a = u(5);
                dVdx = dudx(1);
                dndx = dudx(2);
                dpdx = dudx(3);
                dcdx = dudx(4);
                dadx = dudx(5);












%% Equation editor
% Time-dependence prefactor term
C_V = 0; C_n = 1; C_p = 1; C_c = 1; C_a = 1;
C = [C_V; C_n; C_p; C_c; C_a];

% Flux terms
F_V = (epp(i)/eppmax)*dVdx;
F_n = mu_n(i)*n*(-dVdx + gradEA(i)) + (Dn(i)*(dndx - ((n/Nc(i))*gradNc(i))));
F_p = mu_p(i)*p*(dVdx - gradIP(i)) + (Dp(i)*(dpdx - ((p/Nv(i))*gradNv(i))));
F_c = mu_c(i)*(z_c*c*dVdx + kB*T*(dcdx + (c*(dcdx/(c_max(i) - c)))));
F_a = mu_a(i)*(z_a*a*dVdx + kB*T*(dadx + (a*(dadx/(a_max(i) - a)))));
F = [F_V; mobset*F_n; mobset*F_p; mobseti*K_c*F_c; mobseti*K_a*F_a];

% Electron and hole recombination
% Radiative
r_rad = radset*B(i)*(n*p - ni(i)^2);
% Bulk SRH
r_srh = SRHset*srh_zone(i)*((n*p - ni(i)^2)/(taun(i)*(p + pt(i)) + taup(i)*(n + nt(i))));
% Volumetric surface recombination
alpha = sign_xn(i)*q*dVdx/(kB*T) + alpha0_xn(i);
beta = sign_xp(i)*q*-dVdx/(kB*T) + beta0_xp(i);
r_vsr = SRHset*vsr_zone(i)*((n*exp(-alpha*xprime_n(i))*p*exp(-beta*xprime_p(i)) - ni(i)^2)...
    /(taun_vsr(i)*(p*exp(-beta*xprime_p(i)) + pt(i)) + taup_vsr(i)*(n*exp(-alpha*xprime_n(i)) + nt(i))));
% Total electron and hole recombination
r_np = r_rad + r_srh + r_vsr;

% Source terms
S_V = (q/(eppmax*epp0))*(-n + p - NA(i) + ND(i) + z_a*a + z_c*c - z_a*Nani(i) - z_c*Ncat(i));
S_n = g - r_np;
S_p = g - r_np;
S_c = k_iongen*g - k_ionrec*(c*a-Ncat(i)*Nani(i));
S_a = 0;
S = [S_V; S_n; S_p; S_c; S_a];

        % Remove unused variables - faster and tidier than using conditional
        % statements
        C = C(1:N_variables);
        F = F(1:N_variables);
        S = S(1:N_variables);
    end

%% Initial conditions.
    function u0 = dfic(x)
        i = find(xmesh <= x);
        i = i(end);

        if length(par.dcell) == 1
            % Single layer
            u0_ana = [(x/xmesh(end))*Vbi;
                nleft*exp((x*(log(nright)-log(nleft)))/par.dcum0(end));
                pleft*exp((x*(log(pright)-log(pleft)))/par.dcum0(end));
                dev.Ncat(i);
                dev.Nani(i);];
        else
            % Multi-layered
            u0_ana = [(x/xmesh(end))*Vbi;
                dev.n0(i);
                dev.p0(i);
                dev.Ncat(i);
                dev.Nani(i);];
        end
        u0_ana = u0_ana(1:N_variables);

        % Organise ICs based on number of variables and SOL_IC
        if dficAnalytical
            u0 = u0_ana;
        else
            % Initial conditions taken from input solution
            u0_in = interp1(icx,squeeze(icsol(end,:,:)),x)';
            % If the number of variables has increased then add analytical
            % ICs for missing variables
            if N_variables > length(u0_in)
                % Add initial conditions for new variables from U_ANA
                u0(1:length(u0_in), 1) = u0_in;
                u0(length(u0_in)+1:N_variables, 1) = u0_ana(length(u0_in)+1:N_variables);
            else
                u0 = u0_in;
            end
        end
    end

%% Boundary conditions
% Refer to PDEPE help for the precise meaning of P and Q
% l and r refer to left and right boundaries.
    function [Pl,Ql,Pr,Qr] = dfbc(xl,ul,xr,ur,t)

        switch N_ionic_species
            case 0
                V_l = ul(1);
                V_r = ur(1);
                n_l = ul(2);
                n_r = ur(2);
                p_l = ul(3);
                p_r = ur(3);
                c_l = 0;
                c_r = 0;
                a_l = 0;
                a_r = 0;
            case 1
                V_l = ul(1);
                V_r = ur(1);
                n_l = ul(2);
                n_r = ur(2);
                p_l = ul(3);
                p_r = ur(3);
                c_l = ul(4);
                c_r = ur(4);
                a_l = 0;
                a_r = 0;
            case 2
                V_l = ul(1);
                V_r = ur(1);
                n_l = ul(2);
                n_r = ur(2);
                p_l = ul(3);
                p_r = ur(3);
                c_l = ul(4);
                c_r = ur(4);
                a_l = ul(5);
                a_r = ur(5);
        end

        switch par.V_fun_type
            case 'constant'
                Vapp = par.V_fun_arg(1);
            otherwise
                Vapp = Vapp_fun(par.V_fun_arg, t);
        end

                % Flux boundary conditions for both carrier types.
                % Calculate series resistance voltage Vres
                if Rs == 0
                    Vres = 0;
                else
                    J = e*sp_r*(ur(3) - pright) - e*sn_r*(ur(2) - nright);
                    if Rs_initial
                        Vres = -J*Rs*t/par.tmax;    % Initial linear sweep
                    else
                        Vres = -J*Rs;
                    end
                end

Pl = [-V_l;
  mobset*(-sn_l*(n_l - n0_l));
  mobset*(-sp_l*(p_l - p0_l));
  0;
  0;];

Ql = [0; 1; 1; 1; 1;];

Pr = [-V_r+Vbi-Vapp-Vres;
  mobset*(sn_r*(n_r - n0_r));
  mobset*(sp_r*(p_r - p0_r));
  0;
  0;];

Qr = [0; 1; 1; 1; 1;];


        % Remove unused entries
        Pl = Pl(1:N_variables);
        Pr = Pr(1:N_variables);
        Ql = Ql(1:N_variables);
        Qr = Qr(1:N_variables);
    end
end

